Moving beyond Deletions: Program Simplification via Diverse Program Transformations

To reduce the complexity of software, Developers manually simplify program (known as developer-induced program simplification in this paper) to reduce its code size yet preserving its functionality but manual simplification is time-consuming and error-prone. To reduce manual effort, rule-based approaches (e.g., refactoring) and deletion-based approaches (e.g., delta debugging) can be potentially applied to automate developer-induced program simplification. However, as there is little study on how developers simplify programs in Open-source Software (OSS) projects, it is unclear whether these approaches can be effectively used for developer-induced program simplification. Hence, we present the first study of developer-induced program simplification in OSS projects, focusing on the types of program transformations used, the motivations behind simplifications, and the set of program transformations covered by existing refactoring types. Our study of 382 pull requests from 296 projects reveals that there exist gaps in applying existing approaches for automating developer-induced program simplification. and outlines the criteria for designing automatic program simplification techniques. Inspired by our study and to reduce the manual effort in developer-induced program simplification, we propose SimpT5, a tool that can automatically produce simplified programs (semantically-equivalent programs with reduced source lines of code). SimpT5 is trained based on our collected dataset of 92,485 simplified programs with two heuristics: (1) simplified line localization that encodes lines changed in simplified programs, and (2)checkers that measure the quality of generated programs. Our evaluation shows that SimpT5 are more effective than prior approaches in automating developer-induced program simplification.

==> Makefile <==
all:
	latex main.tex
	bibtex main
	latex main.tex
	latex main.tex
	#dvips -Ppdf -G0 -t a4 icsedraft.dvi
	dvips -Ppdf -G0 -t letter main.dvi
	ps2pdf -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress main.ps main.pdf

.PHONY:clean
clean:
	\rm *.aux *.blg *.bbl *.log


==> backup/ack.tex <==
This research is supported in part by the National Research Foundation, Prime Minister's Office, Singapore under its National Cybersecurity R\&D Program (Award No. NRF2014NCR-NCR001-21) and administered
by the National Cybersecurity R\&D Directorate.

==> backup/anti-macro.tex <==
\newcommand{\antitool}{\emph{anti-patterns}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}
\def\HiLir{\leavevmode\rlap{\hbox to \hsize{\color{red!50}\leaders\hrule height .8\baselineskip depth .5ex\hfill}}}
\def\HiLi{\leavevmode\rlap{\hbox to \hsize{\color{blue!50}\leaders\hrule height .8\baselineskip depth .5ex\hfill}}}

\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\newcommand{\rgenprog}{\emph{rGenProg}}
\newcolumntype{x}[1]{%
{\centering\hspace{0pt}}p{#1}}%
%\newcommand{\evalproj}{seven}
%\newcommand{\evalbugs}{35}


% change the following number when more repairs are generated
\newcommand{\evalproj}{eight}
\newcommand{\evalbugs}{36}
\newcommand{\origge}{54}
\newcommand{\geevalbugs}{42}
\newcommand{\geallevalbugs}{92}

\newcommand{\origspr}{40}
\newcommand{\sprevalbugs}{37}%33
\newcommand{\sprallevalbugs}{85}
%GE total
\newcommand{\geTotSimilar}{8}
\newcommand{\geTotDel}{13}
\newcommand{\geallTotDel}{19}
\newcommand{\geTotLoc}{3}
\newcommand{\geTotSame}{16}
\newcommand{\geallTotSame}{26}
\newcommand{\geTotNoRep}{3}
\newcommand{\geTotSpeed}{0.95}%0.71
\newcommand{\geTotSpeedSame}{1.43}%1.79
\newcommand{\geallTotSpeedSame}{1.42}
\newcommand{\geTotCorrect}{3}
\newcommand{\geTotPla}{40}
\newcommand{\mgeTotCorrect}{2}
\newcommand{\mgeTotVeriYes}{38}
\newcommand{\mgeTotVeriNo}{3}
\newcommand{\mgeTotVeri}{(\mgeTotVeriYes, \mgeTotVeriNo)}
\newcommand{\sprTotCorrect}{12}
\newcommand{\sprTotPla}{24}
\newcommand{\msprTotCorrect}{13}
\newcommand{\msprTotVeriYes}{22}
\newcommand{\msprTotVeriNo}{1}
\newcommand{\msprTotVeri}{(\msprTotVeriYes,\msprTotVeriNo)}
\newcommand{\mgeTotSpace}{39}%1.7 61
\newcommand{\mgeallTotSpace}{40}
\newcommand{\msprTotSpace}{28}%1.53 72
\newcommand{\msprallTotSpace}{28}
%SPR total
\newcommand{\sprTotSimilar}{2}
\newcommand{\sprTotDel}{3}
\newcommand{\sprallTotDel}{10}
\newcommand{\sprTotLoc}{9}
\newcommand{\sprTotSame}{21}
\newcommand{\sprallTotSame}{42}
\newcommand{\sprTotNoRep}{1}
\newcommand{\sprTotSpeed}{1.66}
\newcommand{\sprTotSpeedSame}{1.25}
\newcommand{\sprallTotSpeedSame}{1.69}

\newcommand{\nodeleteallTotSpeedSame}{1.20}




==> backup/antipattern-motivation.tex <==
Although various search-based program repair techniques ~\cite{rsrepair,relifix,genprogae} show promising results in generating a large number of patches, prior studies show that most of these patches are often only plausible but incorrect~\cite{Kali}. Specifically, SPR generates 28 out of 40 (i.e, 70\%) plausible but incorrect patches, while GenProg generates 50 out of 53 (i.e., 94.33\%) plausible patches, for the GenProg benchmarks~\cite{le2012systematic}.
%The difference between plausible and correct patches comes from the definition of ``correctness". Plausible patches simply pass all tests in a given test-suite, while correct patches capture the human intent of patching as shown in a developer given patch.

To better understand the nature of the plausible patches (see Definition~\ref{def:correctness} for definition of plausible patches), we performed a manual inspection on all the machine-generated patches produced by SPR and GenProg (including plausible and correct patches) as well as on the correct developer-provided patches for these bugs. Specifically, we manually analyzed each patch and attempted to answer two questions:
\begin{description}
	\item[Q1:] What makes a given patch plausible? Why is it incorrect (i.e., does not capture the semantics of the developer-provided patch)?
	\item[Q2:] Do the plausible patches, as a whole, share any common syntactic features that explain their ``plausibility'' as well as distinguish them from the pool of correct patches (human as well as machine generated)?
\end{description}
The aim was to find a compact set of syntactic features that are independent of the repair templates used by the tool.
Table~\ref{genprog-spr-anti} shows the results of our manual inspection. Interestingly, our manual inspection identified a set of 14 simple features, shown in the second row of Table~\ref{genprog-spr-anti}, one or more of which appear in \textit{each} of the plausible patches produced by SPR and GenProg and almost none of the correct patches~\footnote{Except for one PHP defect and one Python defect.}.
%except for \texttt{php-309892-309910} and \texttt{python-69783-69784}}.
%XX\% of the plausible SPR patches (row 3) and YY\% of plausible GenProg patches (row 4),
  They correspond to various modifications to the control flow or the data flow of the program.  Each column corresponds to a specific feature and denotes the percentage of plausible patches bearing that feature. Note that our calculation considers the fact that one plausible patch may exhibit several features.
For example, \textit{Delete if-statement} (column 6) deletes an if statement and appears in 28\% of plausible GenProg patches and 10.71\% of plausible SPR patches. Similarly, \textit{Insert Tautology} (column 14) inserts a trivial tautological condition into the program and appears in
7.14\% of the plausible SPR patches but none of the plausible GenProg patches. We further generalize and consolidate these 14 features into 7 transformations, shown in the first row of Table~\ref{genprog-spr-anti}, which we chose to further develop as \tooln\ in our approach.
%\input{antipattern-summary.tex}
%\input{antipattern-problem.tex}


Table~\ref{antipattern-summary} lists the \emph{anti-patterns} that we identified through our manual inspection~\cite{antipattern-book}. In each example patch in Table~\ref{antipattern-summary} and in patches presented throughout the paper, code with a leading ``$\Minus$" denotes statements deleted by the patch, while code with a leading ``$\Plus$" marks statements added. Code without any leading symbol denotes unchanged statements.   

%Hence, it is important to investigate the general characteristic of these patches. We manually examined all plausible but incorrect patches produced by GenProg and SPR for the GenProg benchmarks~\cite{le2012systematic}.

%We choose to include SPR in our experiments to understand the characteristic of patches produced by a pattern-based approach because a subset of SPR ``transformation schemas" (e.g., ``Add Initialization") are essentially templates, as in Pattern-based Automatic program Repair(i.e, PAR)~\cite{PAR}.

%Table~\ref{genprog-spr-anti} shows the recurring characteristic for plausible but incorrect patches produced by GenProg and SPR. The second row in table~\ref{genprog-spr-anti} represents various modifications commonly found in automatically generated patches, while the first row groups together related modifications into specific \tooln.


==> backup/antipattern-problem.tex <==
\begin{table*}
\centering
\caption{Problems in search-based program repairs and the corresponding \tooln\ aim to solve these problems}
\label{antipattern-problem}
%\def\arraystretch{0.95}
\scriptsize
\begin{tabular}{|p{11.5cm}|p{5.4cm}|}
\hline
Problem & \emph{Anti-patterns} \\\hline
\textbf{Weak Oracle.}
Instead of checking for the actual output of a program, developers may validate the outcome of a failing test by relying on the exit status or assertions of the program. Such statements serve as proxies for verifying the correctness of a program, and thus, they should not be manipulated by machine-generated patches. However, such restrictions are not imposed on automatically generated patches. In fact, patches that simply remove such statements may be more preferable for test-driven program repair techniques as they can be generated faster~\cite{Kali}.
 & 
\textbf{\emph{A1: Anti-delete CFG exit node.}} 
 \\\hline
\textbf{Inadequate Test Coverage.} If the program under test has low code coverage, test-driven program repair tools could incorrectly remove a logical block of statements as they are seen as redundant code to the test suite. This may lead to regressions in the patched program~\cite{FSE15paper} & 
\vspace{-0.8\topsep}
 \begin{minipage}[t]{\linewidth}
\begin{itemize}[topsep=0pt,after=\strut,nosep,noitemsep,label={},leftmargin=0mm]
\item\textbf{\emph{A2: Anti-delete Control Statement}}
\item\textbf{\emph{A3: Anti-delete Single-statement CFG}} 
\item\textbf{\emph{A4: Anti-delete Set-Before-If}}
\end{itemize}
 \end{minipage} \\\hline
\textbf{Mask Existing Vulnerabilities.} A patched program may mask previously exposed vulnerability by removing certain branches through implicit data-flow.
&
\textbf{\emph{A4: Anti-delete Set-Before-If}}
\\\hline
\textbf{Non-termination.} Program repair tools may incorrectly remove a loop update statement, causing infinite loop in the patched program. If no timeout is specified, search-based repair tools may spend the entire repair session to validate the patched program. Worst still, such patches could be mistakenly treated as a repair if the test only checks if an error is thrown within a time limit.
 &\textbf{\emph{A5:Anti-delete Loop-Counter Update}}        \\\hline
\textbf{Trivial Patch.} An incorrectly patched program may bypass an important functionality or an error check through insertions of premature exit calls. The worst scenario happens when repair tools produce trivial patches that simply insert return-statements based on the value of the expected output of the failing test (e.g., a trivial patch that insert \texttt{if(test1) return expected-out;})
&\textbf{\emph{A6: Anti-append Early Exit}}         \\\hline
\textbf{Functionality Removal} Repair tools like SPR may produce patches that are semantically equivalent to functionality removal by inserting tautological condition or contradition. A tautology will cause the elimination of the check condition while a contradiction will cause the entire branch to be removed.
& \vspace{-0.8\topsep}
\begin{itemize}[topsep=0pt,noitemsep,label={},leftmargin=0mm]
\item \textbf{\emph{A7: Anti-append Trivial Conditions}} 
\end{itemize}\\\hline
\end{tabular}
\vspace*{-0.9\baselineskip}
\end{table*}


==> backup/antipattern-summary.tex <==
\begin{table*}
\centering
\caption{Our proposed set of \tooln\ with examples that illustrate the usage of each antipattern}
\label{antipattern-summary}
\small
\begin{tabular}{|p{6cm}|p{11cm}|}
\hline
\emph{Anti-patterns} & Example \\\hline
\textbf{\emph{A1: Anti-delete CFG exit node.}}
This pattern disallows removal of return statements, exit calls, functions with the word ``error" (i.e., ignoring letter case), and assertions. 

&\textbf{Ex1:} The example below shows a patch generated by GenProg for \texttt{libtiff-8f6338a-4c5a9ec}. The patch removes the erroneous exit call.
                %\begin{minipage}{0.47\textwidth}
                    %\vspace{4 mm}
             \setbox0=\hbox{\begin{lstlisting}[belowcaptionskip=0pt,belowskip=0pt,caption=Example patch for Anti-delete CFG exit node,label={lst:antideleteret}]
static void BadPPM(char* file) {
    fprintf(stderr, "%s: Not a PPM file.\n", file);
^$\Minus$^    exit(-2);
}       \end{lstlisting}}\mbox{}\box0
\\\hline
\textbf{\emph{A2: Anti-delete Control Statement}} 

This pattern disallows removal of control statements, e.g., if-statements, switch-statements, and loops.
& \textbf{Ex2:} The example below shows a patch generated by GenProg for \texttt{php-307931-307934}. The patch removes the whole if-then-else statement that checks for the return value of a function call.
              \setbox0=\hbox{\begin{lstlisting}[belowcaptionskip=0pt,belowskip=0pt,caption=Example patch for Anti-delete Control Statement,label={lst:antideleteblock}]
call_result = call_user_function_ex(...);
^$\Minus$^ if (call_result == SUCCESS && retval != NULL && ...) {
^$\Minus$^    if (SUCCESS == statbuf_from_array(...))
^$\Minus$^        ret = 0;
^$\Minus$^ } else if (call_result == FAILURE) {
^$\Minus$^          php_error_docref(...);
^$\Minus$^        }
\end{lstlisting}}\mbox{}\box0
\\\hline
\textbf{\emph{A3: Anti-delete Single-statement CFG}} 

This pattern disallows deletion of the statement within a CFG node that has only one statement.
&
\textbf{Ex3:} The example below presents a candidate patch generated by GenProg for \texttt{libtiff-90d136e4-4c66680f}. The patch removes the statement that assigns the return value of 1 which indicates a failure.

\setbox0=\hbox{\begin{lstlisting}[belowcaptionskip=0pt,belowskip=0pt,caption=Example patch for Anti-delete Single-statement CFG,label={lst:antideletesingle}]
fail:{
^$\Minus$^ ret = 1;
}        \end{lstlisting}}\mbox{}\box0

\\\hline

\textbf{\emph{A4: Anti-delete Set-Before-If}} 

This pattern disallows deletion of a variable definition if the variable in the definition is used in subsequent if-statement.  
 & \textbf{Ex4:} The example shows a GenProg generated candidate patch for \texttt{libtiff-d13be72c-ccadf48a}. The patch removes the statement that stores the value of the expression \texttt{EstimateStripByteCounts(...)<0}.


            \setbox0=\hbox{\begin{lstlisting}[belowcaptionskip=0pt,belowskip=0pt,caption=Example patch for Anti-delete Set-Before-If,label={lst:antideletesetbeforeif}]
^$\Minus$^ tmp = EstimateStripByteCounts(tif, dir, dircount)<0;
 if(tmp!=0)
   goto bad;
       \end{lstlisting}}\mbox{}\box0
\\\hline
\textbf{\emph{A5:Anti-delete Loop-Counter Update}} 

Although more sophiscated techniques are needed to ensure termination in patched program, we implement an approximation of this pattern by disallowing deletion of an assignment statement inside a loop if the set of variables used in the terminating condition intersects with the set of variables used in the LHS of the assignment statement.
&            \textbf{Ex5:} The example belows shows a patch that delete the increment statement within a loop.
 

\setbox0=\hbox{\begin{lstlisting}[caption=Example: Anti-delete Loop-Counter Update,label={lst:antideletesetinloop}]
while( x> 5)
^$\Minus$^   x++;
\end{lstlisting}}\mbox{}\box0
\vspace{-5mm} \\\hline
\textbf{\emph{A6: Anti-append Early Exit}} 

This pattern disallows insertion of return statement and goto statement at any location except for after the last statement in a CFG node.
&           \textbf{Ex6:} The example shows a SPR's patch for \texttt{php-308262-308315}. The patch adds a conditional return statement before a function call that throws an error.
               \setbox0=\hbox{\begin{lstlisting}[belowcaptionskip=0pt,belowskip=0pt,caption=Example patch for Anti-append Early Exit,label={lst:antiappendearly}]
^$\Plus$^ if ((type != 0))
^$\Plus$^    return;
zend_error((1<<3L),"Uninitialized string offset:",...);
\end{lstlisting}}\mbox{}\box0
  \\\hline
\textbf{\emph{A7: Anti-append Trivial Conditions}} 

This expression-level pattern disallows insertion of trivial conditions. A condition is trivial iff (1) it is either true or false constant (e.g., if (0), if (1)), (2) it is evaluated to true or false by any assignment of the program variables (e.g., if(x || y || !y)), and (3) it is always evaluated to true or false by any values that program variables can take according to results of static analysis (e.g., if(x || y != 0) in which y is initialized).  
& \textbf{Ex7:} The following example shows two SPR patches for \texttt{lighttpd-2661-2662}. The patch in Listing~\ref{lst:antiappendfalse} appends the condition \texttt{!(1)} to the existing condition, which is semantically equivalent to disabling the branch containing the continue statement. The patch in Listing~\ref{lst:antiappendtrue} loosens the original condition with the expression \texttt{1}, which is semantically equivalent to deleting the condition \texttt{(fields->size==0)}.
\begin{lstlisting}[caption=Example patch with contradiction for Anti-append Trivial Conditions,label={lst:antiappendfalse}]
^$\Minus$^if ((fmap[j].key != format->ptr[i + 1]))
^$\Plus$^if ((fmap[j].key != format->ptr[i + 1]) && !(1))
    continue;
\end{lstlisting}
\vspace{-2mm}
\setbox0=\hbox{
\begin{lstlisting}[belowcaptionskip=0pt,belowskip=0pt,caption=Example patch with tautology for Anti-append Trivial Conditions,label={lst:antiappendtrue}]
^$\Minus$^ if ((fields->size == 0)) {
^$\Plus$^ if ((fields->size == 0) || (1)) {
    fields->size = 16;
    fields->used = 0;
    fields->ptr = malloc(fields->size * sizeof(format_field *));
}
\end{lstlisting}}\mbox{}\box0
\\\hline
\end{tabular}
\end{table*}
%\vspace{-10mm}


==> backup/antipattern-text-description.tex <==
Below are the details of each anti-pattern, as well as the specific problems in test-driven program repair
that these anti-patterns aim to solve.

%\begin{description}
      \begin{description}[leftmargin=0cm]
\item[Problem 1: {\it Weak Oracle.}] Instead of checking for the actual output of a program, developers may validate the outcome of a failing test by relying on the exit status or assertions of the program. Such statements serve as proxies for verifying the correctness of a program, and thus, they should not be manipulated by automatically generated patches. However, such restrictions are not imposed on automatically generated patches. In fact, patches that simply remove such statements may be more preferable for test-driven program repair techniques as they can be generated faster~\cite{Kali}.
    \item[\textbf{Solution 1:} {\it Anti-delete CFG exit node}] This pattern disallows removal of return statements, exit calls, functions with the word ``error" (i.e., ignoring letter case), and assertions.
              \item[Ex. 1:] The example below shows a patch generated by GenProg for \texttt{libtiff-8f6338a-4c5a9ec}. The patch removes the erroneous exit call.\\
                \begin{minipage}{0.47\textwidth}
                    %\vspace{4 mm}
                    \begin{lstlisting}[caption=Example patch for Anti-delete CFG exit node,label={lst:antideleteret}]
static void BadPPM(char* file) {
    fprintf(stderr, "%s: Not a PPM file.\n", file);
^$\Minus$^    exit(-2);
}        \end{lstlisting}
                    %\vspace{2 mm}
                \end{minipage}
    \end{description}
\vspace{-1.5mm}
  \begin{description}[leftmargin=0cm]
\item[Problem 2: {\it Inadequate Test Coverage.}] If the program under test has low code coverage, test-driven program repair tools could incorrectly remove a logical block of statements as they are seen as redundant code to the test suite. This may lead to regressions in the patched program~\cite{FSE15paper}.
 \item[\textbf{Solution 2a:} {\it Anti-delete Control Statement.}] This pattern\\ disallows removal of control statements, e.g., if-statements, switch-statements, and loops.
            \item[Ex. 2a:] The example below shows a patch generated by GenProg for \texttt{php-307931-307934}. The patch removes the whole if-then-else statement that checks for the return value of a function call.\\
                \begin{minipage}{0.47\textwidth}
                    %\vspace{4 mm}
                    \begin{lstlisting}[caption=Example patch for Anti-delete Control Statement,label={lst:antideleteblock}]
call_result = call_user_function_ex(...);
^$\Minus$^ if (call_result == SUCCESS && retval != NULL && Z_TYPE_P(retval) == IS_ARRAY) {
^$\Minus$^    if (SUCCESS == statbuf_from_array(...))
^$\Minus$^        ret = 0;
^$\Minus$^ } else if (call_result == FAILURE) {
^$\Minus$^          php_error_docref(NULL TSRMLS_CC, E_WARNING, "%s::" USERSTREAM_STAT " is not implemented!",
^$\Minus$^          us->wrapper->classname);
^$\Minus$^        }
\end{lstlisting}
                    %\vspace{2 mm}
                \end{minipage}
%        \end{description}
\vspace{-2mm}
%\begin{description}\item[Rationale] To prevent indirect deletion of CFG blocks since the deletion of the only statement within a CFG block will result in an empty CFG node.
\item[\textbf{Solution 2b:} {\it Anti-delete Single-statement CFG.}] This pattern disallows deletion of the statement within a CFG node that has only one statement.
            \item[Ex. 2b:] The example below presents a candidate patch generated by GenProg for \texttt{libtiff-90d136e4-4c66680f}. The patch removes the statement that assigns the return value of 1 which indicates a failure.\\
                \begin{minipage}{0.47\textwidth}
                    %\vspace{4 mm}
                    \begin{lstlisting}[caption=Example patch for Anti-delete Single-statement CFG,label={lst:antideletesingle}]
fail:{
^$\Minus$^ ret = 1;
}        \end{lstlisting}
%\vspace{2 mm}
\end{minipage}
\end{description}
\vspace{-2mm}
    \begin{description}[leftmargin=0cm]
\item[Problem 3: {\it Mask Existing Vulnerabilities.}] A patched program may mask previously exposed vulnerability by removing certain branches through implicit data-flow.
\item[\textbf{Solution 3:} {\it Anti-delete Set-Before-If.}] This pattern disallows deletion of a variable definition if the variable in the definition is used in subsequent if-statement
           \item[Ex 3:] The example shows a GenProg generated candidate patch for \texttt{libtiff-d13be72c-ccadf48a}. The patch removes the statement that stores the value of the expression \texttt{EstimateStripByteCounts(...)<0}.\\
                \begin{minipage}{0.47\textwidth}
                    \begin{lstlisting}[caption=Example patch for Anti-delete Set-Before-If,label={lst:antideletesetbeforeif}]
^$\Minus$^ tmp = EstimateStripByteCounts(tif, dir, dircount)<0;
 if(tmp!=0)
   goto bad;
       \end{lstlisting}
%\vspace{2 mm}
\end{minipage}
\end{description}
\vspace{-2 mm}
   \begin{description}[leftmargin=0cm]
\item[Problem 4: {\it Non-termination.}] Program repair tools may incorrectly removes loop update statement, causing infinite loop in the patched program. If no timeout is specified, search-based repair tools may spend the entire repair session to validate the patched program. Worst still, such patches could be mistakenly treated as a repair if the test only checks if an error is thrown within a time limit.
\item[\textbf{Solution 4:} {\it Anti-delete Loop-Counter Update}] Although \\more sophiscated techniques are needed to ensure termination in patched program, we implement an approximation of this pattern by disallowing deletion of an assignment statement inside a loop if the set of variables used in the terminating condition intersects with the set of variables used in the LHS of the assignment statement.
            \item[Ex 4:] The example belows shows a patch that delete the increment statement within a loop.\\
                \begin{minipage}{0.47\textwidth}
                    \begin{lstlisting}[caption=Example: Anti-delete Loop-Counter Update,label={lst:antideletesetinloop}]
while( x> 5)
^$\Minus$^   x++;
\end{lstlisting}
%\vspace{2 mm}
\end{minipage}
\end{description}
\vspace{-1.5mm}
 \begin{description}[leftmargin=0cm]
    \item[Problem 5: {\it Trivial Patch.}] An incorrectly patched program may bypass an important functionality or an error check through insertions of premature exit calls. The worst scenario happens when repair tools produce trivial patches that simply insert return-statements based on the value of the expected output of the failing test (e.g., a trivial patch that insert \texttt{if(test1) return expected-out;})
\item[\textbf{Solution 5:} {\it Anti-append Early Exit.}] This pattern disallows insertion of return statement and goto statement at any location except for after the last statement in a CFG node.
           \item[Ex. 5:] The example shows a SPR's patch for \texttt{php-308262-\\308315}. The patch inserts a conditional return statement before a function call that throws an error.\\
                \begin{minipage}{0.47\textwidth}
                    \begin{lstlisting}[caption=Example patch for Anti-append Early Exit,label={lst:antiappendearly}]
^$\Plus$^ if ((type != 0))
^$\Plus$^    return;
zend_error((1<<3L),"Uninitialized string offset:",...);
\end{lstlisting}
%\vspace{2 mm}
\end{minipage}
\end{description}

 \begin{description}[leftmargin=0cm]
 \item[Problem 6: {\it Functionality Removal.}] Repair tools like SPR may produce patches that are semantically equivalent to functionality removal by inserting tautological condition or contradition. A tautology will cause the elimination of the check condition while a contradiction will cause the entire branch to be removed.
\item[\textbf{Solution 6:} {\it Anti-append Trivial Conditions}] This\\ expression-level pattern disallows insertion of trivial conditions. We define trivial conditions as (1) conditions that evaluates to either tautology (always true) or contradictions (always false) or (2) complex conditions with part of the condition being a tautology or a contradiction.
               \item[Ex 6:] The following example shows two SPR patches for \texttt{lighttpd-2661-2662}. The patch in Listing~\ref{lst:antiappendfalse} appends the condition \texttt{!(1)} to the existing condition, which is semantically equivalent to disabling the branch containing the continue statement. The patch in Listing~\ref{lst:antiappendtrue} loosens the original condition with the expression \texttt{1}, which is semantically equivalent to deleting the condition \texttt{(fields->size==0)}.\\
                \begin{minipage}{0.46\textwidth}
                    \begin{lstlisting}[caption=Example patch with a contradiction for Anti-append Trivial Conditions,label={lst:antiappendfalse}]
^$\Minus$^if ((fmap[j].key != format->ptr[i + 1]))
^$\Plus$^if ((fmap[j].key != format->ptr[i + 1]) && !(1))
    continue;
\end{lstlisting}
\vspace{-2mm}
\begin{lstlisting}[caption=Example patch with a tautology for Anti-append Trivial Conditions,label={lst:antiappendtrue}]
^$\Minus$^ if ((fields->size == 0)) {
^$\Plus$^ if ((fields->size == 0) || (1)) {
    fields->size = 16;
    fields->used = 0;
    fields->ptr = malloc(fields->size * sizeof(format_field *));
}
\end{lstlisting}

%\vspace{2 mm}
\end{minipage}
\end{description}
\vspace{-3.5mm}
%\end{description}
%=======
%\subsection{Control-flow Based Anti-patterns}
%\label{sec:CntrlFlwAntPtrns}
%
%\begin{lstlisting}[float, caption= Example for Control-flow anti-pattern CF1]
%static void usage(void) {
%        ...
%    exit(-1);
%        ...
%}
%\end{lstlisting}
%
%\begin{lstlisting}[float, caption= Example for Control-flow anti-pattern CF2-1]
%        ...
%if (computeInputPixelOffsets(crop, image, &offsets))  {
%        TIFFError ("getCropOffsets", "Unable to compute crop margins");
%        return (-1);
%}
%        ...
%\end{lstlisting}
%
%\begin{lstlisting}[float, caption= Example for Control-flow anti-pattern CF2-2]
%         ...
%  if ((COMP_UNSET == dc->comp) && !(1))
%          ...
%\end{lstlisting}
%
%\begin{lstlisting}[float, caption= Example for Control-flow anti-pattern CF3]
%if (tif->tif_dir.td_fieldsset[1] & 1UL) {
%tmp___29 = TIFFWriteDirectoryTagShortPerSample(...);
%if (! tmp___29) { goto bad; }
%return (1);
%...
%}
%\end{lstlisting}
%
%\subsection{Data-flow Based Anti-patterns}
%\label{sec:DataFlwAntPtrns}
%
%\begin{lstlisting}[float, caption= Example for Data-flow anti-pattern DF1]
%tmp = EstimateStripByteCounts(tif, dir, dircount) < 0;
%if(tmp!=0)
%    goto bad;
%        ...
%bad:
%        ...
%\end{lstlisting}
%
%
%
%\begin{lstlisting}[float, caption= Example for Data-flow anti-pattern DF2]
%while(x>5){
%    x++;
%}
%\end{lstlisting}
%>>>>>>> fla


==> backup/antirule-my.tex <==
We refer to the seven transformations, identified through our case study, as \emph{anti-patterns} and use them to identify and filter invalid patches that are commonly produced by search-based program repair techniques. 

In the following examples, and in patches presented throughout the paper, code with a leading ``$\Minus$" denotes statements deleted by the patch, while code with a leading ``$\Plus$" marks statements added. Code without any leading symbol denotes unchanged statements.


Below are the details of each anti-pattern:
\begin{description}
      \begin{description}\item[Problem] Instead of checking for the actual output of a program, developers may validate the outcome of a failing test by relying on the exit status or assertions of the program. Such statements serves as proxies for verifying the correctness of a program and thus, they should not be manipulated by automatically generated patches. However, such restrictions are not imposed on automatically generated patches. In fact, patches that simply remove such statements may be more preferable for test-driven program repair techniques as they can be generated faster~\cite{Kali}. 
    \item[\textbf{Solution:} {\it Anti-delete CFG exit nodes}] This pattern disallows deletion of return statements, exit calls, functions that have the word ``error" (i.e., ignoring letter case), and assertions. 
              \item[Example] The example below shows a patch generated by GenProg for \texttt{libtiff-8f6338a-4c5a9ec}. The patch removes the erroneous exit call.\\
                \begin{minipage}{0.45\textwidth}
                    %\vspace{4 mm}
                    \begin{lstlisting}[caption=Example patch for Anti-delete CFG exit nodes,label={lst:antideleteret}]
static void BadPPM(char* file) {
    fprintf(stderr, "%s: Not a PPM file.\n", file);
^$\Minus$^    exit(-2);
}        \end{lstlisting}
                    %\vspace{2 mm}
                \end{minipage}

        \end{description} 
  \begin{description}\item[Problem] As search-based program repair techniques do not imposed any restriction on the test coverage of a given program, automated tools could accidentally treat a logical block of statements to be redundant code. 
 \item[\textbf{Solution:} {\it Anti-delete Control Statement}] This pattern disallows deletion of control statements, including if-statements, switch-statements and loops.
    
            \item[Example] The example below shows a patch generated by GenProg for \texttt{php-307931-307934}. The patch removes the whole if-then-else statement that checks for the return value of a function call.\\
                \begin{minipage}{0.4\textwidth}
                    %\vspace{4 mm}
                    \begin{lstlisting}[caption=Example patch for Anti-delete Control Statement,label={lst:antideleteblock}]
call_result = call_user_function_ex(NULL, &us->object, &func_name, &retval, 0, NULL, 0, NULL TSRMLS_CC);
^$\Minus$^ if (call_result == SUCCESS && retval != NULL && Z_TYPE_P(retval) == IS_ARRAY) {
^$\Minus$^    if (SUCCESS == statbuf_from_array(retval, ssb TSRMLS_CC))
^$\Minus$^        ret = 0;
^$\Minus$^ } else {
^$\Minus$^        if (call_result == FAILURE) {
^$\Minus$^          php_error_docref(NULL TSRMLS_CC, E_WARNING, "%s::" USERSTREAM_STAT " is not implemented!",
^$\Minus$^          us->wrapper->classname);
^$\Minus$^        }
^$\Minus$^ }\end{lstlisting}
                    %\vspace{2 mm}
                \end{minipage}

        \end{description} 
\item[\textbf{Solution 1:} {\it Anti-delete Single-statement CFG}] This pattern disallows deletion of the statement within a CFG block that has only one statement.
    \begin{description}\item[Rationale] To prevent indirect deletion of CFG blocks since the deletion of the only statement within a CFG block will result in an empty CFG node.                
            \item[Example] The example below presents a candidate patch generated by GenProg for \texttt{libtiff-90d136e4-4c66680f}. The patch removes the statement that assigns the return value of 1 which indicates a failure.\\
                \begin{minipage}{0.46\textwidth}
                    %\vspace{4 mm}
                    \begin{lstlisting}[caption=Example patch for Anti-delete Single-statement CFG blocks,label={lst:antideletesingle}]
fail:{
^$\Minus$^ ret = 1;  
}        \end{lstlisting}
%\vspace{2 mm}
\end{minipage}
\end{description} 
\item[\textbf{Solution 2:} {\it Anti-delete Set-Before-If}] This pattern disallows deletion of a variable definition if the variable in the definition is used in subsequent if-statement
    \begin{description}\item[Rationale] To prevent the disabling of branches through implicit data-flow because disabling of branches is semantically equivalent to deleting a CFG blocks. 
            \item[Example] The example shows a GenProg generated candidate patch for \texttt{libtiff-d13be72c-ccadf48a}. The patch removes the statement that stores the value of the expression \texttt{EstimateStripByteCounts(...) < 0}.\\
                \begin{minipage}{0.46\textwidth}
                    \begin{lstlisting}[caption=Example patch for Anti-delete Set-Before-If,label={lst:antideletesetbeforeif}]
^$\Minus$^ tmp = EstimateStripByteCounts(tif, dir, dircount) < 0;
 if(tmp!=0)
   goto bad;
       \end{lstlisting}
%\vspace{2 mm}
\end{minipage}
\end{description} 
   \begin{description}
\item[Problem] Patches that
 such patches could be mistakenly treated as a repair if the test only checks if a particular error message is thrown within a time limit.

To prevent patches that contain infinite loops. Note that such patches could be mistakenly treated as a repair if the test only checks if a particular error message is thrown within a time limit.
\item[\textbf{Anti-pattern 5:} {\it Anti-delete Set-Inside-Loop}] This pattern disallows deletion of set instruction inside a loop if the variable used in the terminating condition is used in the set instruction.  
            \item[Example] The example belows shows a patch that delete the increment statement within a loop.\\
                \begin{minipage}{0.46\textwidth}
                    \begin{lstlisting}[caption=Example patch for Anti-delete Set-Inside-Loop,label={lst:antideletesetinloop}]
while( x> 5)
^$\Minus$^   x++;
\end{lstlisting}
%\vspace{2 mm}
\end{minipage}
\end{description} 
\item[\textbf{Anti-pattern 6:} {\it Anti-append Early Exit}] This pattern disallows insertion of return statement and goto statement at any location except for after the last statement in a CFG block
    \begin{description}\item[Rationale] To prevent skipping the statements that capture the symptoms of a bugs through premature exit.
            \item[Example] The example shows a patch generated by SPR for \texttt{php-308262-308315}. The patch inserts a conditional return statement before an function call that throws an error.\\
                \begin{minipage}{0.46\textwidth}
                    \begin{lstlisting}[caption=Example patch for Anti-append Early Exit,label={lst:antiappendearly}]
^$\Plus$^ if ((type != 0))
^$\Plus$^    return;
zend_error((1 << 3L), "Uninitialized string offset: %ld", (*dim).value.lval);
\end{lstlisting}
%\vspace{2 mm}
\end{minipage}
\end{description} 
\item[\textbf{Anti-pattern 7:} {\it Anti-append Trivial Conditions}] This \\expression-level pattern disallows insertion of trivial conditions. We define trivial conditions as (1) conditions that evaluates to either tautologies or contradictions; or (2) conditions that cause other clauses in the entire conditions to be tautologies or contradictions.   
    \begin{description}\item[Rationale] A tautology will result in disabling of the check conditions while a contradiction will result in disabling of branches.  
            \item[Example] The following example shows two SPR patches for \texttt{lighttpd-2661-2662}. The patch in listing~\ref{lst:antiappendfalse} appends the condition \texttt{!(1)} to the existing condition, which is semantically equivalent to disabling the branch containing the continue statement. The patch in listing~\ref{lst:antiappendtrue} loosen the original condition with the expression \texttt{1}, which is semantically equivalent to deleting the check condition \texttt{(fields->size == 0)}.\\
                \begin{minipage}{0.46\textwidth}
                    \begin{lstlisting}[caption=Example patch with a contradiction for Anti-append Trivial Conditions,label={lst:antiappendfalse}]
^$\Minus$^if ((fmap[j].key != format->ptr[i + 1])) 
^$\Plus$^if ((fmap[j].key != format->ptr[i + 1]) && !(1))
    continue;
\end{lstlisting}
\begin{lstlisting}[caption=Example patch with a tautology for Anti-append Trivial Conditions,label={lst:antiappendtrue}]

^$\Minus$^ if ((fields->size == 0)) {
^$\Plus$^ if ((fields->size == 0) || (1)) {
    fields->size = 16;
    fields->used = 0;
    fields->ptr = malloc(fields->size * sizeof(format_field *));
}
\end{lstlisting}

%\vspace{2 mm}
\end{minipage}
\end{description} 





\end{description}
%=======
%\subsection{Control-flow Based Anti-patterns}
%\label{sec:CntrlFlwAntPtrns}
%
%\begin{lstlisting}[float, caption= Example for Control-flow anti-pattern CF1]
%static void usage(void) {
%        ...
%    exit(-1);
%        ...
%}
%\end{lstlisting}
%
%\begin{lstlisting}[float, caption= Example for Control-flow anti-pattern CF2-1]
%        ...
%if (computeInputPixelOffsets(crop, image, &offsets))  {
%        TIFFError ("getCropOffsets", "Unable to compute crop margins");
%        return (-1);
%}
%        ...
%\end{lstlisting}
%
%\begin{lstlisting}[float, caption= Example for Control-flow anti-pattern CF2-2]
%         ...
%  if ((COMP_UNSET == dc->comp) && !(1))
%          ...
%\end{lstlisting}
%
%\begin{lstlisting}[float, caption= Example for Control-flow anti-pattern CF3]
%if (tif->tif_dir.td_fieldsset[1] & 1UL) {
%tmp___29 = TIFFWriteDirectoryTagShortPerSample(...);
%if (! tmp___29) { goto bad; } 
%return (1);
%...
%}
%\end{lstlisting}
%
%\subsection{Data-flow Based Anti-patterns}
%\label{sec:DataFlwAntPtrns}
%
%\begin{lstlisting}[float, caption= Example for Data-flow anti-pattern DF1]
%tmp = EstimateStripByteCounts(tif, dir, dircount) < 0;
%if(tmp!=0)
%    goto bad;
%        ... 
%bad:
%        ...
%\end{lstlisting}
%
%
%
%\begin{lstlisting}[float, caption= Example for Data-flow anti-pattern DF2]
%while(x>5){
%    x++;
%}
%\end{lstlisting}
%>>>>>>> fla


==> backup/background.tex <==

We present our technique in the context of \textit{search-based program repair} systems, also referred to as ``generate-and-validate" systems in the literature~\cite{SPR-long}. Search-based repair currently represents the one of the most popular and scalable class of automatic program repair approaches. 

For such systems the repair problem consists of a buggy program and a test-suite, with at least one failing test-case that witnesses the bug. The goal of the repair is to modify the program so that it passes all the test-cases. The test-suite acts a \textit{repair specification}, defining the desired behavior of the program, albeit incompletely. The repair system uses a set of \textit{repair schemas} or templates, each typically comprising a local, syntactic modification to the program. The repair starts with a fault localization or repair-site localization step that provides a ranked list of suspicious program locations where a repair could be effected.
The repair tool searches the repair space defined by a single or multiple, successive applications of the repair schemas at each of the repair sites, validating each candidate repair by running the test-suite, till a \textit{plausible} repair passing all the test-cases is found or the search times out. 

Search-based repair approaches face two major challenges. The first is the incredibly large search space, even when restricting the repair to single-line modifications, and the substantial cost of running the test-suite to validate each candidate repair. To alleviate this problem, repair tools may navigate the search space using genetic algorithms~\cite{le2012systematic}, random search~\cite{rsrepair}, or deterministic heuristic search strategies~\cite{SPR-long}, among others. This also influences the choice of repair templates which can range from generic, syntactic code transformations~\cite{le2012systematic, SPR-long} to more elaboratore repair templates derived from human-written patches~\cite{PAR}. Further, repair approaches use a variety of ``smarts" when instantiating candidate repairs to prune candidate repairs that are likely to violate the repair specification, i.e., not pass the test-suite.

A second, relatively less studied, challenge is the incompleteness of the repair specification and its consequence on the quality of repairs. Test-suites, while readily available in most software development projects, are not intended to be repair specifications and are, by their very nature, incomplete. Thus, it is unsurprising that the vast majority of repairs generated by search-based repair tools are far from correct, if not outright wrong~\cite{Kali}. In this work we address this problem. Specifically, we propose the use of a small, set of \textit{anti-patterns} that can be used to reject potentially useless repairs even before they are validated by the test-suite, much less given to the human developer to scrutinize.


==> backup/conclusions.tex <==
In this paper, we proposed integrating \tooln\ to search-based program repair. Our experimental results show that by enforcing \tooln, we produce patches with more pleasant properties, such as patches that delete less functionality, and localize better. Tools integrated with \tooln\ also could generate patches faster due to repair space reduction. A recent study~\cite{ICSE2016} shows the abundance of plausible patches and sparsity of correct patches --- thereby arguing for rich specifications (beyond test-suites) to guide the repair process. Our results indicate that our \tooln, while they are not correctness specifications, form one such set of
specifications whose enforcement can improve patch quality.

%While we choose to enforce all \tooln\ in our integration with repair tools to achieve maximum pruning capability, our integrations provide the flexibility to control the repair space pruning by disabling specific anti-pattern. A study on the trade-off between the efficiency of patch generation and the resulting patch quality is left as future work.

While in this work we explicitly specified a set of anti-patterns as prohibited code transformations, in future, it is feasible to implicitly specify anti-patterns as selected ``code smells".
Thus, during the repair search, any program modification that produces a program with a bad code smell could be effectively prohibited.


Our work opens the possibility of adapting the idea of \tooln\ to other search-based software engineering activities beyond program repair. For example, specific code \tooln\ identifying energy hot-spots may be employed for energy reduction.




In future, we are unlikely to have programming environments that automatically patch all errors without sufficient intervention or domain knowledge. Meanwhile, it might be possible to have programming environments, which attempt to patch programs so as to pass a given test-suite and point the developers to likely error locations and likely fixes. Our proposal of \tooln\ is a step in this direction.





%, and we
%envision that enforcing \tooln\ will be useful for making meaningful patch suggestions to the developer.


 %due to the effectiveness of \tooln\ under the presence of weak oracle (as discussed in ~\ref{sec:genprog-eval}).
%In future, test-suites and \tooln\ specifications, could be further strengthened by other specifications such as models derived by specification mining to further direct repair.

% Our results on mGenProg and mSPR show that our \tooln\ could lead search-based program repair tools to patches that localizes better and patches that removes less functionality. Tools integrated with \tooln\ also could generate patches faster due to our repair space reduction.


==> backup/correctpatchtable.tex <==
\begin{table*}[]
\small
\centering
\caption{Patch Correctness Analysis Result on mGenProg and mSPR}
\label{correct-sum}
\scalebox{0.81}{
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{|l|r|r|r|r|r|r|r|}
%\setlength{\tabcolsep}{0.3em}
\begin{tabular}{lrrrrrrrr}
%\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Subjects} & \multicolumn{2}{c}{GenProg} & \multicolumn{2}{c}{mGenProg} & \multicolumn{2}{c}{SPR} & \multicolumn{2}{c}{mSPR} \\
\cline{2-9}
 & Correct & Plausible & Correct & Plausible & Correct & Plausible & Correct & Plausible \\
\hline
coreutils & 0 & 9 & 0 & 9 & 0 & 11 & 0 & 11 \\  
findutils & 0 & 11 & 0 & 10 & 0 & 9 & 0 & 9 \\
grep & 0 & 9 & 0 & 9 & 0 & 11 & 0 & 11 \\
make & 0 & 5 & 0 & 5 & 0 & 3 & 0 & 3\\ 
\hline \hline
php & 2 & 17  &1 &18 & 8 & 9 & 9 & 8  \\
libtiff & 0 & 16 & 0 & 13 &1 & 4 &1 & 3  \\
python & 1 & 0 & 1 & 0 & 1 & 2 & 1& 2 \\
gmp & 0 & 0 & 0 & 0 & 1 & 1 & 1 & 1 \\
gzip & 0 & 1 & 0 & 1 & 1 & 1 & 1 & 1 \\
wireshark & 0 & 3 & 0 & 3 & 0 & 4  & 0 & 4  \\
fbc & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
lighthttpd & 0 & 2 & 0 & 2 & 0 & 4 & 0 & 4  \\
\hline \hline
Total &0+3=3 & 34+39=73 & 0+2=2 & 33+37=70 &0+12=12 & 34+25=59 & 0+13=13 &34+23=57\\
%Total/Average &3 & 32 & 1 & 31 &12 & 24 & 13 &22\\
\hline
\end{tabular}
}
\vspace*{-0.9\baselineskip}
\end{table*}


==> backup/discussion.tex <==
\begin{description}[leftmargin=0cm]
\item[Patch Quality] 
Our experimental results show that our \tooln\ are able to guide both mGenProg and mSPR in producing patches that localizes better and removes less lines of code. Based on our manual inspection, we think that patches that are able to isolate the correct lines yet not semantically equivalent are still useful as they can serve as repair hints for developers. Meanwhile, producing patches that removes less functionalities reduces the potential destructive effects of generated patches under the presence of weak oracles~\cite{Kali}. SPR generates patches that removes functionality by generation of trivial conditions. Inserting trivial conditions could similarly lead to deletion of functionalities, including deletions of branches and deletions of check conditions. When the condition synthesis engine of mSPR fails to generate nontrivial conditions, the repair engine proceed to modify other potential buggy locations, which may potentially lead to the patches being applied to more precise location compared to the human patch. With our integration of \tooln, our results show that mSPR is still able to generate patches that contain nontrivial conditions. Such nontrivial conditions can also provide hints to developers in generating the correct conditions. 
Our patch analysis results also show that \tooln\ could lead mGenProg in generating patches that localizes the correct buggy function. We attribute the success of this improvement to the \emph{Anti-delete CFG exit nodes} pattern which aims to remove patches that merely remove the symptoms of bugs because statements that captures the symptoms of bugs are usually ranked high by the statistical fault localization step. This improvement also suggests the possibility of using mGenProg as a fix localizing tool that pinpoints the location in which the correct repair needs to be applied.  \\
\hspace{1mm} Our \tooln\ integration achieves greater improvement of patch quality on mGenProg compared to mSPR. We think that this difference is due to the fact that SPR is innately restricted by its set of transformation schemas, which contain transformations that are often used in human patches.
\item[Patch Correctness] Table~\ref{correct-sum} demonstrates that enforcing anti-patterns does not necessarily lead to patches which are exactly equivalent to the human patch. This is not entirely unexpected. Our repair method is driven by a suite of test cases, and aims to pass the test-suite while not inserting any of the anti-patterns. It frees the developer from providing different human patch patterns for different defect classes, exception types, vulnerabilities, et al. Nevertheless, mSPR still generates one more correct repair compared to SPR, while mGenProg generates one plausible repair that involves removing a branch from the original program.  Our further analysis of the bug reports associated with the one case where mGenProg fails to generate the correct repair reveals that although the SPR's correct patch analysis categorized the GenProg repair for \texttt{php-309892-309910}\footnote{https://bugs.php.net/bug.php?id=54454} as a correct repair, the patch was later reverted by the PHP developers because the patch will actually break other functionalities in PHP. In this case, mGenProg repair that deletes less lines of code compared to GenProg's patch may be more preferable.%(2) the correct repair for \texttt{python-69783-69784}\footnote{http://bugs.python.org/issue11930} is issued by Python developers to remove a deprecated functionality. This analysis suggests that \tooln\ is less effective when the repairs involve either deletions that may potentially cause future defects or functionality changes. 
\item[No Repair] Although previous evaluation of search-based repairs~\cite{genprogae} focuses on measuring the total number of successful repair, our results show that mGenProg and mSPR actually produces less number of successful repairs compared to GenProg and SPR. This is because some of the plausible patches produced by GenProg and SPR are actually nonsensical patches that are eliminated by our \tooln. In this case, producing less plausible patches could save the time spent on manual filtering of nonsensical patches which will be subsequently rejected by human developers.
\item[Improvement over no-del-GenProg] Table~\ref{ge-nodelete-sum} shows that GenProg with \tooln\ produces patches of better quality and faster than GenProg that simply prohibits deletions.  
\item[Speedup] Table~\ref{ge-sum} and~\ref{spr-sum} clearly show that by enforcing \tooln, we produce plausible patches faster due to the repair space reduction shown in Table~\ref{tab:repairred}. Overall, we obtain a higher speedup in mSPR compared to mGenProg. This difference could be due to the larger number of invalid patches within the repair space of SPR. We are able to achieve the significant time reduction because we do not explore large parts of the repair space (i.e., greater repair space reduction). One conceptual argument against the idea of \tooln\ may be that it will make the repair search unduly inefficient. Our results show that it is not so. Indeed, the anti-patterns aid us to skip ``irrelevant" parts of the repair space (i.e., repairs that causes undesirable behavior such as the deletion of the symptoms of bugs). 
\item[Weak Proxies] Our experiments for SPR and mSPR use the updated proxies in ~\cite{Kali}  which modify the test harness and the developer test script for \texttt{php} and \texttt{libtiff}. In contrast, we reuse the weak proxies for our experiments on GenProg and mGenProg. If we compare the first two rows of Table~\ref{ge-sum} and Table~\ref{spr-sum} in which different set of proxies are used, we realize that having a stronger proxy does not prevent SPR from generating patches that are semantically equivalent to deletion of functionalities (as indicated in ``Delete Less" and "Better condition" column). This illustrates the fact that our \tooln\ do not require the presence of strong proxies to be effective.
\item[Restrictiveness of \tooln] Another conceptual argument against the idea of \tooln\ may be that the \tooln\ will be overly restrictive and will rule out any repair in many cases, whereas if an existing search-based tool produces some repair it still helps the developer to some extent. Again, our results show that \tooln\ are not overly restrictive, and in the few cases where it ruled out any repair, indeed no valid repair existed.
\item[Implication] Table~\ref{ge-sum} and~\ref{spr-sum} show that by enforcing \tooln, we produce patches with more pleasant properties, such as patches which delete less functionality, patches which localizes better, et al. Thus, we envision that enforcing \tooln\ is useful for making meaningful patch suggestions to the developer. Looking forward several decades from now, we are unlikely to have programming environments which automatically patch all errors without sufficient intervention or domain knowledge. Meanwhile, it might be possible to have programming environments, which attempt to patch programs so as to pass a given test-suite, and in the attempt point the developer to likely error locations and likely fixes. Our proposal of \tooln\ is a step in this direction.
\end{description}
%THINK:should deletion be allowed?
%SpeedUp in terms of operator for SPR
%describe no repair cases in details


==> backup/evaluation.tex <==
%\vspace*{-.1cm}

We compare the effectiveness of \tooln\ on GenProg and SPR using two sets of benchmarks: (1) the CoREBench benchmarks~\cite{corebench} and (2) the GenProg benchmarks~\cite{le2012systematic}. We use the CoREBench benchmarks for the evaluation set because it contains real errors in widely used C programs.
Although our manual inspection for deriving anti-patterns in Section~\ref{sec:prevalence} was based on plausible patches from the GenProg benchmarks,
this study used just \textit{one} generated patch per buggy program. A recent study has shown that the typical repair search space for these bugs contains up to thousands of plausible patches~\cite{ICSE2016}. Thus, we feel it is still meaningful to study the impact of \tooln\ on the complete repair space of these bugs. %MUKUL - paraphrased.
%Though we have previously demonstrated the prevalence of \tooln\ on the GenProg benchmarks in section~\ref{sec:prevalence}, we still include them in our evaluation because it is important to investigate the effect of \tooln\ on the entire repair search space, as the prevalence of \tooln\ has only been observed for one generated patch per buggy program.
Our evaluation studies the following research questions:
\begin{description}
\item[RQ1] How do \tooln\ affect the quality of patches generated by search-based program repair tools?
\item[RQ2] How many nonsensical patches can our \tooln\ eliminate to reduce manual inspection costs?
\item[RQ3] When our modified tools produce the same patch, what is the speedup that we achieve?
\item[RQ4] How does the use of \tooln\ compare to an approach that simply prohibits deletion?
\end{description}
%\vspace*{-\baselineskip}

%The first question (RQ1) evaluates the effect of our modifications on the quality of the generated patches. The second question (RQ2) compares the repairability of both the original tools and the modified tools. The last question accesses the effectiveness of \tooln\ in reducing the time taken when the generated patch is the same for both the original tools and the modified tools.
%\vspace*{-.5\baselineskip}
%\vspace*{-\baselineskip}

\input{gesummarytable.tex}
\begin{table}[!ht]
\centering
%\vspace{1mm}
\caption{\small Subject Programs and Their Basics Statistics}
\scalebox{0.75}{
%\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|r|r|}
\hline
Subjects & Description & kLoC & Tests \\ \hline
coreutils & File, Shell and Text manipulation Utility & 83.1 & 4772 \\
findutils & Directory Searching Utility & 18.0 & 1054 \\
grep & Pattern Matching Utility & 9.4 & 1582 \\
make & Program executable generation utilities & 35.3 &528 \\ \hline \hline
php & Programming Language & 1046 & 8471 \\
libtiff & Image Processing Library & 77 & 78 \\
python & Programming Language & 407 & 35 \\
gmp & Math Library & 145 & 146 \\
gzip & Data Compression Utility & 491 & 12 \\
wireshark & Network Packet Analyzer & 2814 & 63 \\
fbc & Compiler & 97 & 773 \\
lighthttpd & Web Server & 62 & 295 \\ \hline
\end{tabular}
}
\label{tab:ownstat}
%\vspace{1mm}
\end{table}

\vspace*{-0.7\baselineskip}
\subsection{Experimental Setup}\label{sec:setup}
%\input{sprsummarytable.tex}
We evaluate the effects of \tooln\ on 49 defects from the CoREBench benchmarks and at least \sprevalbugs\ defects from the GenProg benchmarks. %The experiments ran are performed on a best-effort basis.
We exclude some versions in our evaluation due to specific technical difficulties, such as benchmarks that require specific system configurations to be built. Specifically, we exclude 21 defects from the CoREBench benchmarks. For the GenProg benchmarks, we manage to reproduce the bugs for \geevalbugs\ defects in the original GenProg experiment and \sprevalbugs\ defects in the original SPR experiments.
%We exclude unfixable program versions that were reported in the original experiments of GenProg and SPR due to limited resources. According to the original GenProg AE results\footnote{http://dijkstra.cs.virginia.edu/genprog/resources/genprog-ase2013-results.zip}, 54 bugs are repairable, we only manage to reproduce the bugs for \geevalbugs\ cases. In the original SPR experiments\footnote{http://rhino.csail.mit.edu/spr-rep/spr-result/}, \origspr\ bugs are repaired, we only manage to reproduce bugs for \sprevalbugs\ of them.

Table~\ref{tab:ownstat} lists information about these subjects. The first four rows of the table list the details for the four CoREBench subjects while the remaining rows show relevant statistics about the GenProg subjects. For each bug, we run GenProg, mGenProg, SPR and mSPR to produce repairs. %Note that we reuse the weak proxies used in the original GenProg experiments for our evaluation of GenProg and mGenProg since we aim to measure the effectiveness of \tooln\ under the presence of week oracles~\cite{Kali}. Since SPR distribution comes with improved proxies, we use the existing modified proxies for the evaluation of SPR and mSPR.

Many of our \tooln\ block functionality deletion, so it is natural to ask if the same effect could be achieved by simply disallowing deletion in repair. To answer RQ4, we implement a customized version of GenProg, called dGenProg, where we disallow the usage of the deletion mutation operator.
%We disallow the usage of the deletion mutation operator in GenProg AE (we called this dGenProg) to stimulate a customized version of GenProg that simply prohibits deletion and use this as a baseline for comparison.
We reuse the same parameters listed in previous work~\cite{le2012systematic} for running GenProg. One significant difference is that we switch to the deterministic adaptive search algorithm (AE)~\cite{genprogae} to control potential randomness. Each run of GenProg, mGenProg, dGenProg, SPR, and mSPR terminates either after all candidate repairs have been evaluated or when a patch is found (i.e., each tool runs to completion without timeout). All experiments for GenProg, mGenProg, and dGenProg were performed by distributing the load on 20 virtual machines with single-core Intel Xeon 2.40GHz processor and 19GB of memory. All experiments for SPR and mSPR were performed on a 12-core Intel Xeon E5-2695 2.40Ghz processor and 408GB of memory.
%(i.e., we allow each tool to run to completion without time limit) or when a patch is found.

After collecting all the repairs, we manually inspect each of these patches and compare the quality of patches generated by GenProg versus mGenProg, mGenProg versus dGenProg, and SPR versus mSPR.
\begin{mydef}\label{def:patch-quality}
We measure the quality of patches generated by search-based repair tools using the criteria defined below:
\begin{description}
\item[(Q1) Same Patch.] A generated repair is considered ``Same Patch" if both the original tool and the modified tool generate exactly the same repair.
\item[(Q2) Localizes Correct Line.] A generated repair is considered ``Localizes Correct Line" if both the generated patch and the human patch generate repairs that modify the same line. For example, we categorize the mGenProg patch in Listing~\ref{lst:correctGenProg} as ``Localizes Correct Line".
\item[(Q3) Localizes Correct Function but Incorrect Line.] A generated repair is considered a patch that localizes the correct function if both the generated patch and the human patch modify statements within the same function.
\item[(Q4) Removes Less Functionality.] A generated repair is considered a repair that removes less functionality if the repair removes or skips over (e.g., by inserting return) fewer lines of source code from the original program.
\item[(Q5) No Repair.] We label a benchmark as ``No Repair" when the original tool generates a repair but the modified tool has iterated through the entire repair space and produce no final patch.
\end{description}
\end{mydef}
\input{correctpatchtable.tex}
\emph{We categorize the patch quality of each repair according to the order listed above (i.e, we first check if a patch is ``Same Patch" and only categorize a patch as ``Removes Less Functionality" if it does not satisfy other more preferable criteria (e.g, ``Localizes Correct Function but Incorrect Line"). We eliminate the potential discrepancies on categorization by ensuring that each defined criteria can be measured through comparisons of the syntactic differences between two patches.}
%Each of the defined criteria measures only the syntactic modifications of the given patches to eliminate the potential discrepancies on categorization.} 

%As the deletions in mSPR are achieved through generation of trivial conditions, we identify a mSPR generated patch as ``Removes Less Functionality" compared to SPR if mSPR generates patches (1)  modifies other locations that causes less functionality removal; (2) uses other transformation schemas (e.g., replace statement and insert memory initialization), while SPR's patches use trivial conditions.

Each column in Tables~\ref{ge-sum},~\ref{spr-sum} and~\ref{ge-nodelete-sum} corresponds to the criteria defined above. The ``Others" column denotes the cases where the patch does not fulfill any of the defined criteria. Numbers in the last row in Tables~\ref{ge-sum}, \ref{spr-sum}, and \ref{ge-nodelete-sum} are of the form $x+y=z$, where $x$ represents the number of patches in the CoREBench benchmarks, $y$ denotes the number of patches in the GenProg benchmarks, and $z$ is the total number of patches in both benchmarks.


We also manually classify and compute the number of correct repairs and the number of plausible repairs.

\begin{mydef} \label{def:correctness}
We use the definition below for our patch correctness analysis:
\begin{description}
\item[Correct Repair.] A repair $r$ is a \emph{correct} repair if (1) $r$ passes all test cases in the test suite and (2) $r$ is semantically equivalent to the repair issued by the developer.
\item[Plausible Repair.] A repair $r$ is a \emph{plausible} repair if (1) $r$ passes all test cases in the test suite but (2) $r$ is \textbf{not} semantically equivalent to the repair issued by the developer.
%\item[Verified Repair] A repair $r$ is a \emph{verified} repair if (1) $r$ passes all test cases in the test suite, (2) does not violate any anti-patterns, and (3) $r$ is \textbf{not} semantically equivalent to the repair issued by the developer
\end{description}
\end{mydef}

\subsection{Evaluation on CoREBench benchmarks}

The first four rows of table~\ref{ge-sum}, ~\ref{spr-sum}, ~\ref{tab:repairred}, and ~\ref{ge-nodelete-sum} show the evaluation results for the CoREBench benchmarks.
\subsubsection{Patch Quality (RQ1)}
Table~\ref{ge-sum} shows that both GenProg and mGenProg produce the same patch for 10 defects in the CoREBench benchmarks. mGenProg could localize the correct line in 7 more defects than GenProg.
%while GenProg could only localize the correct function but incorrect line in 12 defects in the CoREBench benchmarks.
mGenProg also generates patches that remove less functionality in 7 defects.

Table~\ref{spr-sum} shows that both SPR and mSPR produce the same patch in 17 defects. mSPR localizes the correct line in 2 more defects than SPR. For 7 defects, mSPR generates patches that removes less functionality.

Table~\ref{correct-sum} shows the overall patch correctness analysis results for GenProg, mGenProg, SPR, and mSPR for each subject. GenProg generates 34 plausible patches while mGenProg produces 33 plausible patches for the CoREBench benchmarks. Specifically, mGenProg does not produce any repair for \texttt{findutils-e8bd5a2c-66c536b} because the patch violates our \tooln. Both SPR and mSPR generate 34 plausible patches for the CoREBench benchmarks.

%localizes the correct function, while mGenProg does not generate any repair for this defect because the patch generated by GenProg violates our \tooln.



\begin{description}[leftmargin=0cm,font=\itshape]
\item[Improvement on fix localization.] Our results show that \tooln\ could lead both mGenProg and mSPR to producing patches that localize either the correct line or the correct function. \emph{Anti-pattern}-enhanced techniques may achieve this improvement because \tooln\ may filter all invalid repairs on a given location, forcing fixes to be generated at other locations. We claim that the ability to localize more precisely is important because when the repair tools fail to generate the correct repair, the next best thing is to check whether they can still generate hints that may lead developers to the repair faster.
%When search-based repair tools generate plausible but incorrect patches, the integration with \tooln\ could help repair tools to pinpoints more accurately the location in which the correct repair needs to be applied.
%We attribute the success of this improvement to the \emph{Anti-delete CFG exit nodes} pattern which aims to remove patches that merely remove the symptoms of bugs because statements that captures the symptoms of bugs are usually ranked high by the statistical fault localization step. When search-based repair tools generate plausible but incorrect patches, the integration with \tooln\ could help repair tools to pinpoints more accurately the location in which the correct repair needs to be applied.
\item[Less functionality removal.] Under the presence of weak oracles~\cite{Kali}, search-based repair tools may generate patches that pass the test suite by removing untested functionality. Our results shows that \tooln\ help in producing patches that remove less functionality and thus reduce the potential destructive effects of generated patches.
%SPR generates patches that removes functionality by inserting trivial conditions. Inserting trivial conditions could similarly lead to deletion of functionalities, including deletions of branches and deletions of check conditions. When the condition synthesis engine of mSPR fails to generate nontrivial conditions, the repair engine proceed to modify other potential buggy locations, which may potentially lead to the patches being applied to more precise location compared to the human patch.
\item[Comparison between mGenProg and mSPR.] Our \tooln\ integration achieves greater improvement of patch quality on GenProg compared to SPR.
We think that this difference may be due to SPR being innately restricted by its set of transformation schemas, which contain transformations that are often used in human patches.
\item[Predominance of Plausible Patches.] Both GenProg and SPR do not generate any correct patch for the CoREBench benchmarks. One possible explanation is that the defects in the CoREBench have higher error complexity than other benchmarks. Thus more substantial patches are required to fix the errors in these benchmarks~\cite{corebench}. These results also agree with our earlier observation (in Section~\ref{sec:prevalence}) that there is a clear predominance of plausible but incorrect patches among all automatically generated patches.
%\item[General Implication] Table~\ref{ge-sum} and~\ref{spr-sum} show that by enforcing \tooln, we produce patches with more pleasant properties, such as patches which delete less functionality, patches which localizes better, et al. Thus, we envision that enforcing \tooln\ is useful for making meaningful patch suggestions to the developer. Looking forward several decades from now, we are unlikely to have programming environments which automatically patch all errors without sufficient intervention or domain knowledge. Meanwhile, it might be possible to have programming environments, which attempt to patch programs so as to pass a given test-suite, and in the attempt point the developer to likely error locations and likely fixes. Our proposal of \tooln\ is a step in this direction.
\end{description}


\begin{center}
\vspace*{-0.5\baselineskip}

\ovalbox{\begin{minipage}{8cm}
\centering
RQ1: \tooln\ direct repair tools towards generating patches that pinpoint the buggy location more accurately. \emph{Anti-patterns} also reduce the potential destructive effect of automatically generated patches by producing patches that remove less functionality.
\end{minipage}}
%\vspace*{-0.5\baselineskip}
\end{center}

\subsubsection{Reducing Manual Inspection Cost (RQ2)}

SPR may produce multiple patches in one repair session due to the use of batch compilation and its staged repair algorithm. Given several candidate repairs, developers need to manually inspect and verify each individual patch.

%\begin{table}[!ht]

%\begin{tabular}{lrr}
%\multirow{2}{*}{Subjects} & \multicolumn{2}{c}{Number of Patches} \\ \cline{2-3}
% & SPR & mSPR \\ \hline
%grep & 20 & 17 \\
%find & 31 & 19 \\
%make & 15 & 6 \\
%coreutils & 21 & 12 \\ \hline\hline
% & 87 & 54 \\ \hline
%\end{tabular}
%\end{table}


Figure~\ref{fig:number-patch} shows the total number of patches generated by SPR versus mSPR for the CoREBench subjects. As SPR and mSPR can produce multiple patches for a given bug, Figure~\ref{fig:number-patch} reports the total number of patches, while the data in Tables~\ref{ge-sum},~\ref{spr-sum} and~\ref{correct-sum} uses a single, best patch (according to the order in Definition~\ref{def:patch-quality}) among all generated patches for a particular bug.
 Overall, SPR generates 87 patches while mSPR only generates 54 patches. Our patch analysis reveals that all 33 additional patches generated by SPR (not generated by mSPR) are indeeed plausible but incorrect patches.

\begin{figure}[!h]
\centering
\begin{tikzpicture}[scale=0.64]
\begin{axis}[
xtick=data,
axis y line=left,
symbolic x coords={coreutils,findutils,grep,make},
x tick label style={font=\small,text width=1.1cm,align=center},
, ylabel=Number of Patches,
nodes near coords,
enlargelimits=true,
ybar]
\addplot[] coordinates {(coreutils,21) (findutils, 31) (grep,20) (make,15)};
\addplot[fill] coordinates {(coreutils,12) (findutils, 19) (grep,17) (make,6)};
\legend{SPR,mSPR}
\end{axis}
\end{tikzpicture}
\caption{\small Number of Patches Found by SPR vs. mSPR}
\label{fig:number-patch}
\end{figure}



\begin{description}[leftmargin=0cm,font=\itshape]
\item[Discussion on Number of Plausible Patches.] Though \\prior evaluation of search-based repair~\cite{genprogae} focuses on measuring the number of successful repairs, our results show that mSPR actually produces less number of candidate repairs than SPR because some of the plausible patches produced by SPR are actually nonsensical patches that are eliminated by our \tooln. Producing less plausible patches could save the time spent on manual filtering of invalid patches, which would eventually be rejected by developers.
\end{description}


\begin{center}
\vspace*{-0.5\baselineskip}
\ovalbox{\begin{minipage}{8cm}
\centering
RQ2: \emph{Anti-patterns} reduce manual inspection cost by eliminating nonsensical candidate repairs.
\end{minipage}}
%\vspace*{-0.5\baselineskip}
\end{center}


\subsubsection{Speedup (RQ3)}

%\subsubsection{Repair Time Speedup}
The ``Average Speedup (Same Patch)'' column in Tables~\ref{ge-sum}, \ref{spr-sum}, and \ref{ge-nodelete-sum} denotes the average speedup obtained when we only considered the subjects where both the original tool and the modified tool produce the same patch. We use the formula below for our speedup calculation (\emph{Repair Time} is defined as the time taken for a repair to be generated):
\begin{equation}
\resizebox{0.4\textwidth}{!}{%
$Repair\ Time\ Speedup=\frac{Original\ Repair\ Time}{Modified\ Repair\ Time}$
}
\end{equation}
%In general, mGenProg obtain an average repair time speedup of \geTotSpeed x considering all patches (i.e., including the case where both mGenProg and GenProg produce the same patches and when both produce different patches).

When GenProg and mGenProg produce the same patch, mGenProg obtain an average repair time speedup of 1.39x while mSPR obtain an average repair time speedup of 1.78x, for the CoREBench benchmarks.
%\subsubsection{Repair Space Speedup}

%\vspace*{-\baselineskip}
\begin{table}[!ht]
%\vspace*{-\baselineskip}
\centering
\caption{Subject Programs and Repair Space Reduction Results for mGenProg and mSPR}
\label{tab:repairred}
\scalebox{0.7}{
\begin{tabular}{lcc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Subject}} & \multicolumn{2}{c}{Repair Space Reduction(\%)} \\ \cline{2-3}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{mGenProg} & \multicolumn{1}{c}{mSPR} \\\hline %\cline{1-1}
coreutils & 43 & 22 \\
findutils & 47 & 19 \\
grep & 38 & 32\\
make & 37& 36\\\hline \hline
php & 37 & 20 \\
libtiff & 43 & 61 \\
python & 31 & 26 \\
gmp & - & 9\\
gzip & 43 & 31 \\
wireshark & 42  & 35 \\
fbc & - & - \\
lighthttpd & 41 & 15 \\ \hline \hline
Average & 41, 40, 40 & 27, 28, 28\\ \hline
%Average & \mgeTotSpace & \msprTotSpace \\ \hline
\end{tabular}
}
\vspace*{-\baselineskip}
\end{table}



Table~\ref{tab:repairred} shows the overall reduction in the total number of repair candidates generated for mGenProg and mSPR. The last row is of the form $x$, $y$, $z$ where $x$ denotes average for CoREBench subjects, $y$ denotes average for GenProg subjects and $z$ denotes the average for all subjects. We calculate the ``Repair Space Reduction" according to the formula below (where $TotC$ refers to the total number of repair candidates within the entire repair search space):
\begin{equation}
\resizebox{0.42\textwidth}{!}{%
    $Repair\ Space\ Reduction=(1-\frac{Modified\ TotC}{Orig\ TotC})*100$
}
\end{equation}
%\vspace*{-1.8\baselineskip}
On average, mGenProg achieves 41\% repair space reduction compared to GenProg while mSPR obtains 27\% repair space reduction compared to SPR for CoREBench subjects.

\begin{description}[leftmargin=0cm,font=\itshape]
\item[Discussion on Speedup.] Tables~\ref{ge-sum} and~\ref{spr-sum} show that by enforcing \tooln, we produce patches faster due to  repair space reduction shown in Table~\ref{tab:repairred}. One conceptual argument against the idea of \tooln\ may be that it might make the repair search unduly inefficient. These results show that it is not so. In fact, the anti-patterns skip ``irrelevant" parts of the repair space (i.e., repairs that causes undesirable behavior, such as the deletion of the symptoms of a bug).
\end{description}
\vspace*{-0.5\baselineskip}
\begin{center}
\ovalbox{\begin{minipage}{8cm}
\centering
RQ3: \emph{Anti-patterns}\ reduce the overall repair time by pruning significant portion of the repair space.
\end{minipage}}
\end{center}
\input{nodelete.tex}


\subsubsection{Comparison with dGenProg (RQ4)}

Table~\ref{ge-nodelete-sum} shows the results for dGenProg versus mGenProg for the CoREBench benchmarks. While both mGenProg and dGenProg produce 12 same patches, mGenProg localizes better compared to dGenProg in seven more subjects than dGenProg. \emph{Although dGenProg explicitly prohibits deletions, our results show that mGenProg actually removes less functionality in five subjects compared to dGenProg}. Our analysis reveals that dGenProg may produce patches that skip over many source lines of code by introducing early return. For \texttt{make-73e7767f-d584d0c1}, mGenProg localizes the correct line while dGenProg do not produce any repair.

When mGenProg and dGenProg produce the same patch, mGenProg achieves an overall speedup of \nodeleteallTotSpeedSame x over dGenProg in the CoREBench benchmarks.

\begin{description}[leftmargin=0cm,font=\itshape]
\item[Improvement over dGenProg.] Our results on the CoRE\\Bench benchmarks show that GenProg with \tooln\ produce patches of better quality and faster than GenProg that simply prohibits deletions.
\end{description}
%\vspace*{-0.5\baselineskip}
\begin{center}
\ovalbox{\begin{minipage}{8cm}
\centering
RQ4: \emph{Anti-patterns} produce patches of better quality and faster than an tool that simply prohibits deletions.
\end{minipage}}
\end{center}

%\vspace*{-0.2\baselineskip}
\subsection{Evaluation on GenProg benchmarks}\label{sec:genprog-eval}

The 5-12th rows of Tables ~\ref{ge-sum},~\ref{spr-sum},~\ref{tab:repairred}, and~\ref{ge-nodelete-sum} show the experimental results for the GenProg benchmarks. Tables~\ref{ge-sum} and~\ref{spr-sum} illustrate that our \tooln\ achieve similar improvement on patch quality on the GenProg benchmarks. In particular, mGenProg localizes better than GenProg in seven more defects. mGenProg also removes less functionality in 12 defects. In contrast, mSPR removes less functionality than SPR in three defects on GenProg benchmarks.

Table~\ref{correct-sum} shows that GenProg produces 3 correct repairs and 39 plausible repairs while mGenProg produces two correct repairs and 37 plausible repairs for the GenProg benchmarks. mGenProg does not generate any repair for three subjects due to their violations of \tooln. Instead of producing correct repair as in GenProg, mGenProg only generates plausible repairs for \texttt{php-309892-309910} because the correct repair actually involves deletion of a if-statement, which violates our \emph{Anti-delete Control Statement} pattern. In contrast, mSPR produces one more correct patch than SPR and 23 plausible repairs. Specifically, mSPR produces correct patch for \texttt{php-308262-308315} while SPR only generates plausible patch for this version. For \texttt{libtiff-086036\\-1ba752}, mSPR does not generate any repair while SPR generates patch with trivial condition that disables a branch. As the correct repair for this libtiff defect requires modifications of multiple statements, our analysis reveals that the correct repair is indeed outside of SPR's repair space.

We also achieve similar reduction on repair time on the GenProg benchmarks, as in the CoREBench benchmarks.
%For the GenProg benchmarks, mSPR produces one more correct patch than SPR and 22 plausible repairs. Specifically, mSPR produces correct patch for \texttt{php-308262-30831\\5} while SPR only generates plausible patch for this version. For \texttt{libtiff-086036-1ba752}, mSPR does not generate any repair, while SPR generates patch with trivial condition that disable a branch. As the correct repair requires modifications of multiple statements (as explained in previous paragraph), our manual inspection reveals that the correct repair is indeed outside of SPR's repair space.


%As shown in table~\ref{ge-sum}, both GenProg and mGenProg produce the same patch in 16 subjects in the GenProg benchmarks. mGenProg localizes better than GenProg in 7 more subjects (8+3=11 subjects in mGenProg versus 1+3=4 subjects in GenProg), removes less functionality compared to GenProg in 12 subjects in the GenProg benchmarks.  For 2 subjects (i.e., \texttt{libtiff-086036-1ba752}, \texttt{libtiff-3af2\\60-723918}) that we categorize as ``Localizes Correct Function" for GenProg, GenProg generates patches that are applied to the same function as the buggy function (i.e., closer by default since mGenProg does generate), but these patches violate our \tooln\ so mGenProg does not generate any repair for these versions. For the one remaining libtiff version (i.e., \texttt{libtiff-ed4969-8a184d}) that mGenProg does not generate any repair, GenProg generated patch does not satisfy any of criteria listed above so we categorizes this patch as ``Others" in Table~\ref{ge-sum}.

%Table~\ref{spr-sum} shows that both SPR and mSPR generate the same patch in 10 subjects in the GenProg benchmarks. mSPR localize either the correct line or correct function in 7+1=8 subjects while SPR localizes correctly in 1+6=7 subjects. mSPR removes less functionality in 3 subjects in the GenProg benchmarks.
\begin{description}[leftmargin=0cm,font=\itshape]
\item[Restrictiveness of \tooln.] Another conceptual argument against the idea of \tooln\ may be that \tooln\ will be overly restrictive and will rule out any repair in many cases whereas, if an existing search-based tool produces some repair, it still helps the developers to some extent. Our results on the GenProg benchmarks show that \tooln\ are not overly restrictive and, in the few cases where it ruled out any repair, indeed no valid repair existed.
\item[Weak Proxies.] Our experiments for SPR and mSPR use the updated proxies in previous work~\cite{Kali}, which modifies the test harness and the developer test script for \texttt{php} and \texttt{libtiff}. In contrast, we reuse the weak proxies for our experiments on GenProg and mGenProg. We used the weak oracles for GenProg and the strong oracles for SPR because they are provided together with the original tool distribution. If we compare the row 5-6 of Tables~\ref{ge-sum} and~\ref{spr-sum} in which different set of proxies are used, we observe that having a stronger proxy does not
    help SPR substantially in terms of fix localization. Indeed the improvement of mSPR over SPR in terms of localizing the correct line, is similar to the improvement of mGenProg over GenProg.
    %This illustrates that our \tooln\ do not require the presence of strong proxies to be effective.
\end{description}

%\subsubsection{Patch Correctness Analysis (RQ2)}
%In total, GenProg generates 3+32=35 patches with 3 correct repairs and 35 plausible repairs, while mGenProg generates 2 correct repairs and 30 plausible repairs for the GenProg benchmarks. mGenProg does not generate any repair for 3 subjects due to their violations of \tooln. Instead of generating correct repair as in GenProg, mGenProg only generates plausible repairs for \texttt{php-309892-309910} because the correct repair actually involves deletion of a if-statement which violates our \emph{Anti-delete CFG block} pattern.

%For the GenProg benchmarks, mSPR produces one more correct patch than SPR and 22 plausible repairs. Specifically, mSPR produces correct patch for \texttt{php-308262-30831\\5} while SPR only generates plausible patch for this version. For \texttt{libtiff-086036-1ba752}, mSPR does not generate any repair, while SPR generates patch with trivial condition that disable a branch. As the correct repair requires modifications of multiple statements (as explained in previous paragraph), our manual inspection reveals that the correct repair is indeed outside of SPR's repair space.

\begin{description}[leftmargin=0cm,font=\itshape]
\item[Discussion on Patch Correctness.] Our results show that enforcing anti-patterns does not necessarily lead to patches that are exactly equivalent to the human patches. This is not entirely unexpected,
because {\em we only mark a generated patch as correct, if it is near identical to the developer provided patch.} %This is conservative, patches marked as not correct could be semantically equivalent to the developers' provided patches.}
Our repair method is driven by a suite of test cases and aims to pass the test-suite while not inserting any of the anti-patterns. It frees the developers from providing different human patch patterns for different defect classes, exception types, vulnerabilities, etc. Nevertheless, mSPR still generates one more correct repair than SPR while mGenProg generates one plausible repair that removes a branch from the original program.  %Our further analysis of the bug reports associated with the one case where mGenProg fails to generate the correct repair reveals that although the SPR's correct patch analysis categorized the GenProg repair for \texttt{php-309892-309910}\footnote{https://bugs.php.net/bug.php?id=54454} as a correct repair, the patch was later reverted by the PHP developers because the patch actually broke other functionalities in PHP. In this case, mGenProg repair that deletes less lines of code compared to GenProg's patch may be more preferable.
\end{description}
\vspace*{-\baselineskip}

\begin{center}
\ovalbox{\begin{minipage}{0.48\textwidth}
\centering
\emph{Anti-patterns} provides repair space reduction, yet are not overly restrictive.
\end{minipage}}
\end{center}


==> backup/ge-algo.tex <==

\begin{algorithm}[!ht]
%\begin{minipage}{\linewidth}
\caption{\small Search-Based Repair generation algorithm}\label{alg:searchrepairalg}
\setstretch{0.9}
\small
%\KwIn{List of suspicious statements $RankList$ , Set of test suite $T$, Reduced test suite $T_r\ \subseteq\ T$, List of contextual operators $O$, Set of program expression $E$, Period $P$ -- the number of iterations for each location before considering next location}
\KwIn{Fitness function $Fit: Program \rightarrow \mathbb{R}$}
\KwIn{$M$: the transformation functions.}
\KwIn{PopSize: population size}
\KwOut{Patch: a program variant that passes all test cases or $\emptyset$ if failed}
\algorithmfootnote{$Apply(Pop, M)$: apply a mutation operation on a given population.\\$Select(Pop, PopSize, Fit)$ : Select the best variant based on fitness function $Fit$}
            $Pop' \gets initialPopulation(PopSize)$\;
\begin{tcolorbox}[width=0.48\textwidth,colback=white] 
\For{m \textbf{in} M}{
    \If{$\neg isAntipattern(P,m)$}{
        $M' \gets M' \cup m$\;
    }
}
\end{tcolorbox}
\Repeat{$\exists$ Patch in Pop that passes all test cases} {
      $Pop' \gets Apply(Pop, M')$\;
      $Pop' \gets Select(Pop, PopSize, Fit)$\;
}
%\end{minipage}
\end{algorithm}


{
\fontsize{5}{5}\selectfont
\setlength{\textfloatsep}{0.1cm}
\setlength{\floatsep}{0.1cm}
\setstretch{0.9}
\LinesNumberedHidden
\begin{algorithm}[!h]
\scalebox{0.7}{
\begin{minipage}{\linewidth}
\small
%\KwIn{List of suspicious statements $RankList$ , Set of test suite $T$, Reduced test suite $T_r\ \subseteq\ T$, List of contextual operators $O$, Set of program expression $E$, Period $P$ -- the number of iterations for each location before considering next location}
\KwIn{Program $P$: Prog}
\KwIn{Test suite $Suite$: Prog$\rightarrow P(Test)$}
\KwIn{Equivalence relation ~: Prog $\times$ Prog $\rightarrow \beta$}
\KwIn{Edit degree parameter $k:$ $N$}
\KwIn{Edit operator $Edits$~: Prog $\times N$ $\rightarrow P(Prog)$}
\KwIn{Repair strategy $RepairStrat$: P(Prog) $\times Model$ $\rightarrow Prog$}
\KwIn{Test strategy $TestStrat$: P(Test) $\times Model$ $\rightarrow Test$}
\KwOut{Program P'. $\forall t \in$  Suite(P'). P'(t)=true}
$Model \gets \emptyset$\;
$EquivClasses \gets \emptyset$\;
$CandidateRepairs \gets \emptyset$\;
\algorithmfootnote{
  $RepairStrat$ controls the order in which each candidate is considered.
\\$TestStrat$ determines the order in which
tests are presented to P.
\\Note that we uses the same edit degree (i.e., k=1) as in original AE. First-degree edit operations include ``deletion" and "insertion of a statement copied from elsewhere in the same program"
}
\begin{tcolorbox}[width=0.9\textwidth,colback=red!50] 
    \For{$P' \textbf{in} Edits(P,k)$)}{
        \If{$\neg isAntipattern(P')$}{
            $CandidateRepairs \gets P'$\;
    }
}
\end{tcolorbox}
\Repeat{$CandidateRepairs == \emptyset$}{
    $P' \gets RepairStrat(CandidateRepairs,Model)$
    $CandidateRepairs \gets CandidateRepairs \setminus \{P'\}'$\;
    \If{$\neg\exists Previous \in EquivClasses. p' ~ Previous)$}{
            $EquivClasses \gets EquivClasses \cup {P'}$\;
            $TestRemaining \gets Suit(P')$\;
            $TestResult \gets true$\;
    }
    \Repeat{$TestRemaining== \emptyset \lor \neg TestResult$}{
     $t \gets TestStrat(TestRemaining,Model)$\;
     \textbf{let} $TestsRemaining \gets TestsRemaining \setminus \{t\}$\;
     $TestResult \gets P'(T)$\;
     $Model \gets Model \cup {<P', t,TestResult>}$\;
    \lIf{$TestResult$}{
       \Return{P'}
    }
    }
%    //check equivalence repair and evaluate P'
}

\caption{\small mGenProg Repair generation algorithm}
\label{alg:mGenProgrepairalg}
\end{minipage}
}
\end{algorithm}
\setlength{\textfloatsep}{0.1cm}
\setlength{\floatsep}{0.1cm}
}

{\fontsize{5}{5}\selectfont
\setlength{\textfloatsep}{0.01cm}
\setlength{\floatsep}{0.01cm}
\begin{algorithm}[!ht]
%\scalebox{0.7}{
%\begin{minipage}{\linewidth}
\caption{\small mSPR Repair generation algorithm}\label{alg:mSPRrepairalg}

\setstretch{0.9}
\small
%\KwIn{List of suspicious statements $RankList$ , Set of test suite $T$, Reduced test suite $T_r\ \subseteq\ T$, List of contextual operators $O$, Set of program expression $E$, Period $P$ -- the number of iterations for each location before considering next location}
\KwIn{original program <p,n>}
\KwIn{positive and negative test cases NegT amd PosT test, each is a set of pairs <I,O> where I is the test input and O is the expected output}
\KwOut{the repaired program <p' n'> or $\emptyset$ if failed}
\algorithmfootnote{
  $M(<p, n>)$: the transformation functions.
\\
$Exec(<p, n>, I, D)$: runs the program <p, n> on input I given the abstract condition value sequence D.
\\$Test(p, n, NegT, PosT)$ : check if the program <p, n> passes all tests
\\$Flip(R)$: negates the input condition R
}
\begin{tcolorbox}[width=0.48\textwidth,colback=red!50] 
\For{<p',n'> \textbf{in} M(<p, n>)}{
    \If{$\neg isAntipattern(<p',n'>)$}{
        $M' \gets M' \cup <p'n'>$\;
    }
}
\end{tcolorbox}
\For{<p',n'> \textbf{in} M'(<p, n>)}{
        \If{p' contains abstc}{
            $R' \gets \epsilon$\;
            $S' \gets \epsilon$\;
        \For{<I,O> in NegT)}{
            $<O', R, S> \gets Exec(<p',n'>,I,\epsilon)$\;
            $cnt \gets 0$\;
            \While{$O'\not=O$ and $cnt\le10$}{
                \lIf{$cnt = 10$}{
                    $D \gets 1 \circ 1 \circ 1 \circ 1 \ldots$
                }\lElse{
                    $D \gets Flip(R)$
                    }
                $<O', R, S> \gets Exec(<p',n'>,I,D)$\;
                $cnt \gets cnt + 1$\;
            }
            \uIf{$O'\not=O$}{
                    skip to the next candidate <p', n'>;
                }\Else{
                    $R' \gets R' \circ R$\;
                    $S' \gets S' \circ S$\;
                    }
      }
     \For{<I,O> in PosT)}{
               $<O', R, S> \gets Exec(<p',n'>,I,\epsilon)$\;
               $R' \gets R' \circ R$\;
               $S' \gets S' \circ S$\;
     }
     $C \gets {}$\;
     \For{$\sigma$ \textbf{in} $S'$}{ 
         $C \gets C \cup \lbrace (v == const), !(v == const)$ | 
          $\forall v \forall const, such\ that \sigma(v) = const \rbrace$\;
         
     }
    $cnt \gets 0$\;

     \While{$C\not=\emptyset$ and $cnt<20$}{
                let $c \in C$ maximizes $F(R',S', c)$\;
           \begin{tcolorbox}[width=0.48\textwidth,colback=yellow!50]     \If{$\neg isTrivialCondition(c)$}{
                $C \gets C/{c}$\;
                \If{Test(<p'[c/abstc],n'>,NegT)}{
                    \Return{<p'[c/abstc],n'>}
                }
            }
        \end{tcolorbox}
                $cnt \gets cnt + 1$\;
            }

}\Else{
                \lIf{Test($<p',n'>,NegT$)}{
                    \Return{$<p',n'>$}
                }
 
}
}
%\end{minipage}
%}
\end{algorithm}
}


==> backup/genprogtable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{My caption}
\label{my-label}
\scalebox{0.7}{
\begin{tabular}{|l|r|r|r|r|r|r|}
\hline
\multirow{2}{*}{Versions} & \multicolumn{2}{c|}{Better Patch} & \multirow{2}{*}{Closer Location} & \multirow{2}{*}{Same patch} & \multirow{2}{*}{No repair} & \multirow{2}{*}{Time reduction} \\ \cline{2-3}
 & Similar to Correct Patch & Delete less &  &  &  &  \\ \hline
php-bug-307931-307934 &  &  & 1 &  &  & 0.02 \\ \hline
php-bug-309986-310009 &  &  &  &  &  & 0.50 \\ \hline
php-bug-309111-309159 &  &  &  & 1 &  & 1.50 \\ \hline
php-bug-310011-310050 &  &  &  & 1 &  & 1.10 \\ \hline
php-bug-307562-307561 &  &  &  & 1 &  & 1.58 \\ \hline
php-bug-308525-308529 &  &  &  & 1 &  & 1.11 \\ \hline
php-bug-307302-307307 &  & 1 &  &  &  & 2.83 \\ \hline
php-bug-307687-307688 &  &  &  &  &  &  \\ \hline
php-bug-307688-307689 &  &  &  &  &  &  \\ \hline
php-bug-307843-307846 &  &  &  &  &  &  \\ \hline
php-bug-307846-307853 &  &  &  &  &  &  \\ \hline
php-bug-307914-307915 &  &  &  & 1 &  & 2.23 \\ \hline
php-bug-308262-308315 &  &  &  & 1 &  & 1.49 \\ \hline
php-bug-308323-308327 &  &  &  & 1 & 1 & 1.18 \\ \hline
php-bug-308475-308477 &  &  &  &  &  &  \\ \hline
php-bug-308523-308525 &  &  &  & 1 &  & 3.08 \\ \hline
php-bug-309487-309491 &  &  &  & 1 &  & 1.59 \\ \hline
php-bug-309516-309535 &  & 1 &  &  &  & 1.65 \\ \hline
php-bug-309579-309580 &  &  &  &  &  &  \\ \hline
php-bug-309892-309910 &  &  &  & 1 &  & 0.10 \\ \hline
php-bug-309984-309986 &  & 1 &  &  &  & 0.03 \\ \hline
php-bug-310673-310681 &  & 1 &  &  &  & 0.87 \\ \hline
php-bug-311164-311141 &  & 1 &  &  &  & 1.41 \\ \hline
php-bug-311323-311300 &  &  &  &  &  &  \\ \hline
libtiff-bug-5b02179-3dfb33b &  &  &  &  &  & 0.21 \\ \hline
libtiff-bug-d13be72c-ccadf48a &  &  &  &  &  & 0.84 \\ \hline
libtiff-bug-d39db2b-4cd598c &  &  &  & 1 &  & 1.06 \\ \hline
libtiff-bug-01209c9-aaf9eb3 &  &  &  &  &  & 0.94 \\ \hline
libtiff-bug-10a4985-5362170 &  &  &  &  &  & 0.48 \\ \hline
libtiff-bug-0661f81-ac6a583 &  & 1 &  &  &  & 0.51 \\ \hline
libtiff-bug-0860361d-1ba75257 &  &  &  &  & 1 & 0.02 \\ \hline
libtiff-bug-0fb6cf7-b4158fa & 1 &  &  &  &  & 0.23 \\ \hline
libtiff-bug-3af26048-72391804 &  &  &  &  & 1 & 0.02 \\ \hline
libtiff-bug-4a24508-cc79c2b &  &  &  & 1 &  & 0.84 \\ \hline
libtiff-bug-5e6542ee-e779b6cd &  & 1 &  &  &  & 0.89 \\ \hline
libtiff-bug-6f9f4d7-73757f3 &  &  &  & 1 &  & 0.87 \\ \hline
libtiff-bug-829d8c4-036d7bb &  &  &  &  &  &  \\ \hline
libtiff-bug-8f6338a-4c5a9ec &  &  & 1 &  &  & 0.16 \\ \hline
libtiff-bug-90d136e4-4c66680f & 1 &  &  & 1 &  & 0.04 \\ \hline
libtiff-bug-ed4969a-8a184dc &  &  &  &  & 1 & 0.03 \\ \hline
libtiff-bug-ee2ce5b7-b5691a5a & 1 &  &  &  &  & 0.05 \\ \hline
python-bug-69783-69784 &  &  &  & 1 &  & 1.21 \\ \hline
gmp-bug-14166-14167 &  &  &  &  &  &  \\ \hline
gzip-bug-3fe0caeada6aa3-39a362ae9d9b00 &  &  &  & 1 &  & 1.12 \\ \hline
wireshark-bug-37112-37111 &  &  &  &  &  &  \\ \hline
wireshark-bug-37172-37171 & 1 &  &  &  &  & 0.50 \\ \hline
wireshark-bug-37172-37173 & 1 &  &  &  &  & 0.51 \\ \hline
wireshark-bug-37284-37285 & 1 &  &  &  &  & 0.53 \\ \hline
fbc-bug-5458-5459 &  &  &  &  &  &  \\ \hline
Total & 6 & 7 & 2 & 16 & 4 & 0.88 \\ \hline

\end{tabular}
}
\end{table*}



==> backup/gesummarytable.tex <==
\begin{table*}[!ht]
\centering
\small
\caption{Overall Results on GenProg (AE) versus mGenProg (mAE)}
\label{ge-sum}
\setlength{\tabcolsep}{0.25em}
\scalebox{0.88}{
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{rrrrrrrrrrrrr}
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}{@{}c@{}}\\\\\\ Subjects\end{tabular}}} & \multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}{@{}c@{}}\\\\\\  Same Patch\end{tabular}}} & \multicolumn{9}{c}{Different Patch} & \multicolumn{1}{c}{}\\ \cline{3-11} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{}& \multicolumn{4}{c}{Localizes Better} & \multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}{@{}c@{}}\\\\ Less Functionality\\ Removal\end{tabular} }} & \multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}{@{}c@{}}\\\\No Repair\end{tabular}}} & \multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}{@{}c@{}}\\\\Others\end{tabular}}}& \multicolumn{1}{c}{\multirow{1}{*}{\begin{tabular}{@{}c@{}}\\ Average Speedup\end{tabular}}}\ \\ \cline{3-6} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{\begin{tabular}{@{}c@{}} Localizes Correct\\ Line\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}{@{}c@{}} Localizes Correct\\ Function but \\Incorrect Line\end{tabular}} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}    & \multicolumn{1}{c}{\multirow{1}{*}{(Same Patch)}}               \\ \cline{3-6}\cline{8-11} 
 & & \multicolumn{1}{c}{AE}    & mAE    & AE               & mAE               & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{ AE}      & mAE  & \multicolumn{1}{c}{AE}      & mAE & \multicolumn{1}{c}{} \\ \hline \hline
coreutils & 0 & 0 & 0 & 4 & 4 & 5 & 0 & 0 & 5 & 0  & - \\
%general0.58\\
findutils & 4 &  0 & 4 & 2 & 1 & 1 & 0 & 1 & 5 & 0 & 1.11\\
%0.96\\
grep & 4 & 0 & 2 & 3  & 2 & 1 & 0 & 0 & 2 & 0 & 1.30 \\
%1.00 \\
make & 2 & 0 & 1 & 3 & 2 & 0 & 0 & 0  & 0 & 0 & 1.77 \\ \hline \hline
%1.27 \\ \hline \hline
php & 10 & 1 & 1 & 0 & 2 &  6 & 0 & 0 & 8 & 0 & 2.08 \\
libtiff & 3 & 0 & 4 & 3 & 1 & 5 & 0 & 3 & 10 &0& 1.13\\
python & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.98\\
gmp & - & - & - & - & - & - & - & - & - & -& - \\
gzip & 1  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0&1.12 \\
wireshark & 0 & 0 & 3 & 0 & 0 & 0 & 0 & 0 & 3 & 0& - \\
fbc & - & - & - & - & - & - & - & - & - & - &-\\
lighthttpd & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 0 &1 & 0& 1.85 \\\hline \hline
Total &10+16=\geallTotSame&	0+1=1	&7+8=15& 12+3=15&	9+3=12&	7+12=19&0+0=0&	1+3=4&	12+22=34&0+0=0 & 1.39+1.43=\geallTotSpeedSame\\
%Total & 10 & 0 &	7	& 12&	9&	0&	7&	0	&1	&12	&0& 1.33 \\ \hline
%0.95 \\ \hline
\hline
\end{tabular}
}
%\vspace*{-\baselineskip}
\end{table*}
\begin{table*}[!ht]
\small
\centering
\caption{Overall Results on SPR versus mSPR}
\label{spr-sum}
\scalebox{0.88}{
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{rrrrrrrrrrrrr}
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}{@{}c@{}}\\\\\\ Subjects\end{tabular}}} & \multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}{@{}c@{}}\\\\\\  Same Patch\end{tabular}}} & \multicolumn{9}{c}{Different Patch} & \multicolumn{1}{c}{}\\ \cline{3-11} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{}& \multicolumn{4}{c}{Localizes Better} & \multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}{@{}c@{}}\\\\ Less Functionality\\ Removal\end{tabular} }} & \multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}{@{}c@{}}\\\\No Repair\end{tabular}}} & \multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}{@{}c@{}}\\\\Others\end{tabular}}}& \multicolumn{1}{c}{\multirow{1}{*}{\begin{tabular}{@{}c@{}}\\Average Speedup\end{tabular}}}\ \\ \cline{3-6} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{\begin{tabular}{@{}c@{}} Localizes Correct\\ Line\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}{@{}c@{}} Localizes Correct\\ Function but \\Incorrect Line\end{tabular}} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}    & \multicolumn{1}{c}{\multirow{1}{*}{(Same Patch)}}               \\ \cline{3-6}\cline{8-11} 
& & \multicolumn{1}{c}{SPR}    & mSPR    & SPR               & mSPR               & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{SPR}      & mSPR  & \multicolumn{1}{c}{SPR}      & mSPR & \multicolumn{1}{c}{} \\ \hline \hline
coreutils & 6 & 0 & 0 & 2 & 2 & 3 & 0 & 0 & 3 & 0  & 1.56\\
%1.37\\
findutils & 6 &  1 & 2 & 1 & 0 & 1 & 0 & 0 & 1 & 0 & 1.62 \\
%1.43\\
grep & 5 & 0 & 1 & 3  & 3 & 2 & 0 & 0 & 3 & 0 & 2.15\\
%2.31 \\
make & 0 & 0 & 0 & 2 & 2 & 1 & 0 & 0  & 1 & 0 & -\\ \hline \hline
%1.73 \\ \hline \hline
php & 15 & 0 & 2 & 2 & 0 &  0 & 0 & 0 & 0 & 0 & 1.96 \\
libtiff & 2 & 1 & 1 & 1 & 0 & 1 & 0 & 1 & 1 &0& 2.10\\
python & 2 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 1.50\\
gmp & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0& 1.42 \\
gzip & 1  & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 1 & 0&1.08 \\
wireshark & 3 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0&1.85 \\
fbc & - & - & - & - & - & - & - & - & - & - &-\\
lighthttpd & 0 & 0 & 2 & 1 & 0 & 2 & 0 & 0 &3 & 0& - \\\hline \hline
Total & 17+25=\sprallTotSame & 1+1=2 & 3+7=10 & 8+6=14 & 7+1=8 & 7+3=10 & 0+0=0 & 0+1=1 & 8+5=13 & 0+0=0
& 1.78+1.65=\sprallTotSpeedSame \\\hline 
%Total & 17& 1 & 3 & 8 & 7 & 0 & 7 &	0 & 0 & 8 & 0 &	 1.78 \\ \hline
%1.71\\ \hline
\end{tabular}
}
\vspace*{-0.9\baselineskip}
\end{table*}



==> backup/introduction.tex <==
Program simplification techniques have been adopted in many automated tools, including debugging~\cite{ddmin,hammoudi2015use}, test case simplification~\cite{zhang2013practical,ddinput,jiang2017simplydroid}, removing code bloat in genetic programming~\cite{wong2007effects,javed2022simplification}, and improving the understanding of features in neural code intelligence system~\cite{rabin2021understanding}. These techniques are usually inspired by the algorithm in delta debugging~\cite{ddinput} where the redundant parts of the input program are removed with the goal of reducing its source code size, leading to a smaller program which is semantically equivalent (produces the same outputs for a given input) to the original program. A simplified or a smaller program has the benefits of being: (1) easier to understand, (2) easier to maintain, and (3) more efficient to run.

Although program simplification techniques have shown promising results in automatically reducing the program size in many automated tools~\cite{zhang2013practical,ddinput,jiang2017simplydroid,rabin2021understanding,wong2007effects}, it is unclear whether the same technique (i.e., deleting irrelevant parts of the program) is used by software developers when simplifying code by hand (we call this \emph{manual program simplification}). Specifically, there is little to no study on \emph{how do developers simplify code during the software development process}.   


To bridge the gaps between automated program  simplification techniques and manual program simplification used in practice, we present the first study of the manual program simplification techniques used by developers in open-source projects in GitHub. Specifically, our study aims to answer the research questions below:

\smallskip

\noindent
\textit{\textbf{(RQ1) How often do developers simplify a program by performing only deletions of existing program statements?}}

We study how often do developers simplify code by removing irrelevant program statements. 


\textit{\textbf{(RQ2) Beyond mere deletions, what are the common sets of program transformations used by developers for simplifying programs?}}

Our intuition is that \emph{different from existing program simplification techniques that perform mere deletions, there exists many other forms of program transformations used by developers when performing manual program simplification}. Hence, we study the common set of program transformations used in manual program simplification.


Although automated program simplification and manual program simplification shares similar goals of reducing the size of the program while preserving its semantics, our study reveals that: (1) only \todo{x} of the studied programs are simplified using mere deletions, and (2) manual program simplification may involve diverse forms of program transformations (with \todo{most prevalence} being the most prevalent used transformations by software developers). 

As performing manual program simplification can be time-consuming and error-prone, we propose \tooln{}, a novel approach transformer-based that can automatically simplify the given input program to support manual program simplification for developers.

 In summary, we made the following contributions:
\begin{itemize}[leftmargin=*,labelindent=7pt,nosep]
    \item To the best of our knowledge, we conducted the first study of the set of program transformations used by developers in open-source projects when performing manual program simplification. Our study shows that developers may use a diverse form of program transformation beyond mere deletions when simplifying code by hand.
    \item We introduce \tooln{}, a novel transformer-based approach that automatically simplify a given input program. Our key technical insight is that program simplification is a more specific task of the general program transformation task. Hence, our approach leverages existing dataset on program transformation by performing pre-training on the general code transformations tasks and fine-tuning on the specific program simplification. \todo{changes this if not correct}   
     \item We propose \bench{}, a benchmark that contains a set of \numbench{} code simplifying commits across \numprojbench{} open-source Java projects. Our evaluation on \bench{} shows that \tooln{} can automatically simplify code with \truepositive{}\% true positive rate on average. The dataset and the source code for \tooln{} are publicly available at https://github.com/. \todo{add link}
\end{itemize}





==> backup/motivation.tex <==

We illustrate how \tooln\ can improve program repair by showing two examples of fixes in two projects. The first example shows the effect of applying \tooln\ for improvement in fix localization, while the second example demonstrates the benefit of \tooln\ in reducing patch generation time.
%We next introduces the set of anti-patterns used and detailed examples for each anti-pattern.
\begin{figure}[!t]
\centering
\begin{minipage}[b]{0.485\textwidth}
\begin{lstlisting}[caption=Example patch generated by GenProg, label={lst:origGenProg},mathescape]
`// GenProg AE patch for findutils-84aef0ea-07b941b1`
static boolean parse_noop (const struct parser_table* entry, char **argv, int *arg_ptr)
{
  (void) entry;
 ^$\Minus$^ return parse_true(get_noop(), argv, arg_ptr);
}
\end{lstlisting}
\end{minipage}%%
%\hfill
\\
\begin{minipage}[b]{0.48\textwidth}
\begin{lstlisting}[caption=Example patches generated by mGenProg and Findutils developer, label={lst:correctGenProg}]
`// mGenProg patch for findutils-84aef0ea-07b941b1`
static boolean
insert_regex (char **argv, int *arg_ptr, const struct parser_table *entry, int regex_options)
{...
   if (error_message)
     error (1, 0, "%s", error_message);
   (*arg_ptr)++;
^$\Minus$^   our_pred->est_success_rate = estimate_pattern_match_rate(argv[*arg_ptr], 1);
   return true;

`// Developer patch for findutils-84aef0ea-07b941b1`
insert_regex (char **argv, int *arg_ptr, const struct parser_table *entry, int regex_options)
{...
   if (error_message)
     error (1, 0, "%s", error_message);
^$\Minus$^  (*arg_ptr)++;
   our_pred->est_success_rate = estimate_pattern_match_rate(argv[*arg_ptr], 1);
^$\Plus$^  (*arg_ptr)++;
   return true;
 \end{lstlisting}
\end{minipage}
\vspace{-3mm}
\end{figure}


\noindent\textbf{Example 1: Improving fix localization.} Listing~\ref{lst:origGenProg} shows the GenProg patch for \texttt{findutils-84aef0ea-07b941b1}  generated by GenProg. The GenProg patch deletes the only return statement in \texttt{parse_noop(...)}. This patch violates our \emph{Anti-delete CFG exit node} pattern. In contrast, our version of GenProg modified with \tooln, called mGenProg, removes the statement that assigns the return value of \texttt{estimate_pattern_match_rate} to the field \texttt{our_pred->est_success_rate}. Meanwhile, Findutils developer moved the statement \texttt{(*arg_ptr)++} to the location after the problematic statement \texttt{our_pred->est_success_rate=estimate_pattern_match_rate(...);} that throws ``Segmentation fault" error due to out-of-bound access of the \texttt{argv} array (Listing~\ref{lst:correctGenProg}).
We argue that in this example, our mGenProg patch is preferable to GenProg's because (1) mGenProg localizes the correct function compared to the GenProg patch, which is applied inside a completely different function \texttt{parse_noop()}; (2) mGenProg correctly pinpoints the function call that causes the error, while the GenProg patch completely removes the functionality encapsulated by the \texttt{parse_noop()} function. This example shows that \tooln\ can improve fix localization and eliminate nonsensical patches that remove functionality.

\begin{figure}[!Ht]
\centering
\begin{lstlisting}[caption={Example patch generated by GenProg, mGenProg and PHP developers}, label={lst:allGenProg},mathescape]
`// GenProg, mGenProg & Developer patch for php-309111-309159`
if ((p = memchr(s, '?', (ue - s)))) {
    pp = strchr(s, '#');
    if (pp && pp < p) {
^$\Plus$^   if (pp - s) {
^$\Plus$^      ret->path = estrndup(s, (pp-s));
^$\Plus$^      php_replace_controlchars_ex(ret->path, (pp - s));
^$\Plus$^   }
            p = pp;
            goto label_parse;
    }
}
\end{lstlisting}
\end{figure}

\noindent\textbf{Example 2: Accelerating program repair.} Listing~\ref{lst:allGenProg} shows a patch that inserts a conditional statement that can be copied from other places within the same file. While both GenProg and mGenProg generate the patch in listing ~\ref{lst:allGenProg} that is in fact equivalent to the correct patch, mGenProg takes only 13.7 hours compared to 20.6 hours taken by GenProg (i.e., mGenProg achieves a 20.6/13.7 = 1.5x speedup).
Thus, if the correct repair can be found within the repair space, our \tooln\ can serve as a search-space pruning mechanism that reduces the time taken to find the correct repair through filtering of invalid patches.

Table~\ref{antipattern-problem} shows the common problems in the patches generated by search-based program repair tools together with the \emph{anti-patterns} that solve these problems.
\vspace{-1mm}
%\begin{figure}[!Ht]
%\centering
%\begin{lstlisting}[caption={Example patch generated by GenProg, mGenProg and PHP developers}, label={lst:allGenProg},mathescape]
%`// `
%  if ((forever) && !((!((forever) )))) {
%      tail_forever(F, n_files, sleep_interval);
%  }
%\end{lstlisting}
%\end{figure}


==> backup/nodelete.tex <==
\begin{table*}[!ht]
\small
\centering
\caption{Overall Results on mGenProg (mAE) versus dGenProg(dAE)}
\label{ge-nodelete-sum}
\setlength{\tabcolsep}{0.3em}
\scalebox{0.79}{
%\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}{@{}c@{}}\\\\\\ Subjects\end{tabular}}} & \multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}{@{}c@{}}\\\\\\  Same Patch\end{tabular}}} & \multicolumn{9}{c}{Different Patch} & \multicolumn{1}{c}{}\\ \cline{3-11} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{}& \multicolumn{4}{c}{Localizes Better} & \multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}{@{}c@{}}\\\\ Less Functionality\\ Removal\end{tabular} }} & \multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}{@{}c@{}}\\\\No Repair\end{tabular}}} & \multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}{@{}c@{}}\\\\Others\end{tabular}}}& \multicolumn{1}{c}{\multirow{1}{*}{\begin{tabular}{@{}c@{}}\\Average Speedup\end{tabular}}}\ \\ \cline{3-6} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{\begin{tabular}{@{}c@{}} Localizes Correct\\ Line\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}{@{}c@{}} Localizes Correct\\ Function but \\Incorrect Line\end{tabular}} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}    & \multicolumn{1}{c}{\multirow{1}{*}{(Same Patch)}}               \\ \cline{3-6}\cline{8-11} 
& & \multicolumn{1}{l}{dAE}    & mAE    & dAE               & mAE               & \multicolumn{1}{c}{}             & \multicolumn{1}{l}{dAE}      & mAE  & \multicolumn{1}{l}{dAE}      & mAE & \multicolumn{1}{c}{} \\ \hline \hline
coreutils & 4 & 0 & 0 & 1 & 1 & 3 & 0 & 0 & 3 & 0 & 1.80\\
%1.19 \\
findutils & 3 &  0 & 5 & 1 & 1 & 0 & 0 & 0 & 5 & 0 & 1.03 \\
%1.90 \\
grep & 2 & 0 & 1 & 3  & 3 & 2 & 0 & 0 & 4 & 1 & 0.79 \\ 
%20.19 \\
make & 3 & 0 & 1 & 1 & 1 & 0 & 1 & 0  & 0 & 0 & 1.18\\  \hline\hline
%2.27 \\ \hline \hline
Total & 12 & 0	& 7 & 6 & 6 & 5 & 1 & 0 & 12 & 1 & \nodeleteallTotSpeedSame \\ \hline
%6.39\\ \hline
\end{tabular}
}
\vspace*{-\baselineskip}
\end{table*}


==> backup/oldexample.tex <==
\noindent\textbf{Example 2: Generating a better patch.} Listing~\ref{lst:origGenProg} shows the patch for \texttt{84aef0ea-07b941b1}  generated by GenProg. The GenProg patch deletes the entire conditional statement that throws an error if the call to \texttt{computeInputPixelOffsets(...)} fails. Note that this patch violates our \emph{Anti-delete CFG block} pattern. In contrast, our version of GenProg modified with \tooln, called mGenProg, deletes only the statement that assigns the default value of \texttt{res_unit} to the field \texttt{image->res_unit}, essentially avoiding \texttt{image->res_unit} to have the default resolution unit. Meanwhile, the Libtiff developers replace the call to \texttt{TIFFGetFieldDefaulted(...)} by \texttt{TIFFGetField(...)} to achieve a similar goal of avoiding \texttt{image->res_unit} to be assigned the default resolution unit. 
%While both GenProg patch and mGenProg patches involve deletion of statements, we think 
We argue that in this example, our mGenProg patch is preferable to GenProg's because (1) the location in which the mGenProg patch is applied is closer to the buggy location (i.e., inside \texttt{loadImage()}) compared to the GenProg patch which is applied inside a completely different function \texttt{getCropOffsets()}; (2) the GenProg patch only removes the symptoms of the bug, while our mGenProg patch is semantically close to the developer's patch and provides more useful hints in generating the correct patch. This example illustrates that \tooln\ could improve fix localization and eliminate nonsensical patches that merely remove the symptoms of a bug.


\begin{figure}[!t]
\centering
\begin{minipage}[b]{0.485\textwidth}
\begin{lstlisting}[caption=Example patch generated by GenProg, label={lst:origGenProg},mathescape]
`// GenProg AE patch for libtiff-5b02179-3dfb33b`
static int getCropOffsets(struct image_data *image, struct crop_mask *crop, struct dump_opts *dump)
{...
/* Compute pixel offsets if margins or fixed width or length specified */
   if ((crop->crop_mode & CROP_MARGINS) ||
      (crop->crop_mode & CROP_REGIONS) ||                              
      (crop->crop_mode & CROP_LENGTH)  ||
      (crop->crop_mode & CROP_WIDTH)) { 
 ^$\Minus$^  if (computeInputPixelOffsets(crop, image, &offsets)) {
 ^$\Minus$^      TIFFError ("getCropOffsets", "Unable to compute crop margins");  
 ^$\Minus$^      return (-1);
 ^$\Minus$^  }
 ...                                       
 }
}
\end{lstlisting}
\end{minipage}%%
%\hfill
\\
\begin{minipage}[b]{0.48\textwidth}
\begin{lstlisting}[caption=Example patches generated by mGenProg and Libtiff developer, label={lst:correctGenProg}]
`// mGenProg patch for libtiff-5b02179-3dfb33b`
static int loadImage(TIFF* in, struct image_data *image, struct dump_opts * dump, unsigned char **read_ptr)
{ ...
  TIFFGetFieldDefaulted(in, TIFFTAG_RESOLUTIONUNIT, &res_unit); 
  scanlinesize = TIFFScanlineSize(in);
  image->bps = bps;
  image->spp = spp;
  image->planar = planar;
  image->width = width;
  image->length = length;
  image->xres = xres;
  image->yres = yres;
^$\Minus$^ image->res_unit = res_unit;
}
`// Developer patch for libtiff-bug-5b02179-3dfb33b`
static int loadImage(TIFF* in, struct image_data *image, struct dump_opts * dump, unsigned char **read_ptr)
{ ...
^$\Minus$^TIFFGetFieldDefaulted(in, TIFFTAG_RESOLUTIONUNIT, &res_unit);
^$\Plus$^TIFFGetField(in, TIFFTAG_RESOLUTIONUNIT, &res_unit);
  ..
  image->res_unit = res_unit;
}
\end{lstlisting}
\end{minipage}
\end{figure}
\begin{table*}[!ht]
\centering
\caption{Overall Results on mGenProg}
\label{ge-sum}
\scalebox{0.8}{
\begin{tabular}{|l|c|c||c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\multirow{3}{*}{Subjects}} & \multicolumn{2}{c||}{\multirow{2}{*}{Same Patch}} & \multicolumn{7}{c|}{Different Patch} \\ \cline{4-10} 
\multicolumn{1}{|l|}{} & \multicolumn{2}{c||}{} & \multicolumn{2}{c|}{Similar to Human Patch} & \multicolumn{1}{c|}{\multirow{2}{*}{Delete Less}} & \multicolumn{2}{c|}{Closer Location} & \multicolumn{1}{c|}{\multirow{2}{*}{No Repair}} & \multicolumn{1}{c|}{\multirow{2}{*}{Average Speedup}} \\ \cline{2-5} \cline{7-8}
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{Subject} & \multicolumn{1}{c||}{Average Speedup} & \multicolumn{1}{c|}{GenProg} & \multicolumn{1}{c|}{mGenProg} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{GenProg} & \multicolumn{1}{c|}{mGenProg} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}\\ \hline
php & 10 & 2.08 & 1 & 1 & 6 & 0 & 2 & 0 & 1.46 \\
libtiff & 3 & 1.13 & 0 & 4 & 6 & 2 & 1 & 3 & 0.49 \\
python & 1 & 0.98 & 0 & 0 & 0 & 0 & 0 & 0 & 0.98 \\
gmp & - & - & - & - & - & - & - & - & - \\
gzip & 1 & 1.12 & 0 & 0 & 0 & 0 & 0 & 0 & 1.12 \\
wireshark & 0 & 0.00 & 0 & 3 & 0 & 0 & 0 & 0 & 0.51 \\
fbc & - & - & - & - & - & - & - & - & - \\
lighthttpd & 1 & 1.85 & 0 & 0 & 1 & 0 & 0 & 0 & 1.14 \\\hline
% & 16 & 1.79 & 0 & 8 & 13 & 2 & 3 & 3 & 0.71
Total/Average & \geTotSame & \geTotSpeedSame & 1 & \geTotSimilar & \geTotDel & 2 & \geTotLoc & \geTotNoRep & \geTotSpeed \\ \hline
\end{tabular}
}
\end{table*}




==> backup/prevalence-antipattern.tex <==
\begin{table*}
\renewcommand{\arraystretch}{1.2}
\centering
\small
\caption{\small Prevalence of Anti-patterns in Plausible Patches}
\label{genprog-spr-anti}
\setlength{\tabcolsep}{0.24em}
\scalebox{0.69}{
%\resizebox{1.04\linewidth}{!}{%
\begin{tabular}{ccccc|cc|c|c|c|ccc|cc}
%\begin{tabular}{M{1cm}M{1.5cm}M{1.5cm}|M{1.5cm}M{1.5cm}M{1.5cm}M{1.5cm}|M{3.0cm}|M{1.5cm}|M{1.5cm}|M{1.5cm}M{1.5cm}M{1.5cm}|M{1.5cm}M{1.5cm}}
\cline{1-15}
\multicolumn{1}{l}{\multirow{2}{*}{}}  & \multicolumn{4}{c}{Anti-delete CFG exit node} & \multicolumn{2}{c}{Anti-delete Control Statement} & \multicolumn{1}{c}{\begin{tabular}{@{}c@{}}Anti-delete\\Single-statement CFG\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}{@{}c@{}}Anti-delete\\Set-Before-If\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}{@{}c@{}}Anti-delete\\Loop-Counter Update\end{tabular}} & \multicolumn{3}{c}{Anti-append Early Exit}  & \multicolumn{2}{c}{\begin{tabular}{@{}c@{}}Anti-append\\Trivial Conditions\end{tabular}} \\  \cline{1-15} 
\multicolumn{1}{l}{} & \begin{tabular}{@{}c@{}}Delete\\exit\end{tabular} & \begin{tabular}{@{}c@{}}Delete\\return\end{tabular} & \begin{tabular}{@{}c@{}}Delete\\goto\end{tabular} & \begin{tabular}{@{}c@{}}Delete\\error code\end{tabular} & \begin{tabular}{@{}c@{}}Delete\\if-statement\end{tabular} & \begin{tabular}{@{}c@{}}Delete\\loop\end{tabular} &  \begin{tabular}{@{}c@{}} Delete only\\ statement within if\end{tabular} & \begin{tabular}{@{}c@{}}Delete\\condition\end{tabular}          & \begin{tabular}{@{}c@{}}Delete loop \\counter update\end{tabular} & \begin{tabular}{@{}c@{}}Insert \\early return\end{tabular} &\begin{tabular}{@{}c@{}} Insert \\early exit\end{tabular} &\begin{tabular}{@{}c@{}} Insert \\early goto\end{tabular} &\begin{tabular}{@{}c@{}} Insert \\Tautology \end{tabular}             &\begin{tabular}{@{}c@{}} Insert \\Contradiction\end{tabular} \\ \hline \hline
GenProg & 4.00\% & 8.00\% & 2.00\% & 14.00\% & 28.00\% & 6.00\% & 4.00\% & 4.00\% & 2.00\% & 2.00\% & 0\% & 2.00\%  & 0\% & 0\% \\ 
SPR &  0\%  & 7.14\%  & 7.14\% & 14.29\% & 10.71\%  & 21.43\%  & 7.14\% & 7.14\% & 3.57\% & 7.14\%              & 3.57\%            & 3.57\% & 7.14\% & 39.29\% \\ \hline \hline
Average & 2.00\% & 7.57\% & 4.57\% & 14.14\% & 19.36\% & 13.71\% & 5.57\% & 5.57\% & 2.79 \% & 4.57\% & 1.79\% &2.79\% & 3.57\% & 19.65\% \\ \hline
\end{tabular}
}
%\vspace*{-\baselineskip}
\end{table*}


==> backup/repair-patterns.tex <==

\section{Set of Program Transformations for Program Simplication}
\label{sec:pattern}
\begin{table}[]
\addtolength{\tabcolsep}{-3pt}
\centering
\caption{Supported Operators in \droixtool}
\label{oplist}
%\resizebox{\linewidth}{!}{%
\footnotesize
\begin{tabular}{ll}
Operator                        & Description \\
\hline\hline
\multirow{2}{*}{S1: GetActivity-check}  & Insert a condition to check whether the activity containing \\
				         &  the fragment has been created.\\
\hline
				                    		
S2: Retain object                       & Store objects and load them when configuration changes\\
\hline
S3: Replace resource id                 & Replace resource id with another resource id of same type. \\
\hline
\multirow{2}{*}{S4: Replace method}     & Replace the current method call with another method call \\
                                         & with similar name and compatible parameter types. \\
\hline
S5: Replace cast                        & Replace the current type cast with another compatible type. \\
\hline
S6: Move stmt                           & Removes a statement and add it to another location. \\
\hline
S7: Null-check                          & Insert condition to check if a given object is null.\\
\hline
S8: Try-catch                           & Insert try-catch blocks for the given exception.\\
\hline
\end{tabular}%}
\end{table}



%Our manual analysis of Android apps reveals that lifecycle-related crashes and resource-related crashes can be resolved with a generic set of transformations. Accordingly, we have developed 
Our manual analysis of crashes in Android apps identifies eight program transformation operators which are useful for repairing these crashes. Table~\ref{oplist} gives an overview of each operator derived through our analysis. As ``Missing Null-check" is one of the common causes of crashes in Table~\ref{tab:rootcause}, we include this operator (S7: Null-check) in our set of operators. Another frequently used operator (5\%) that fixes crashes that occur across different categories in Table~\ref{tab:rootcause} is inserting exception handler (S8: Try-catch) which we also include into our set of operators. We now proceed to discuss other program transformation operators in Table~\ref{oplist} and the specific reasons of crashes associated with each operator in this section. 
%During our automated repair, these transformation operators will be applied
%repeatedly according to a {\em search strategy}.  

\noindent\textbf{Retain stateful object} Configuration changes (e.g., phone rotation and language) cause activity to be destroyed and recreated which allows apps to adapt to new configuration (transition from \texttt{onDestroy()}$\rightarrow$ \texttt{onCreate()}).  According to Android documentation~\footnote{https://developer.android.com/guide/topics/resources/runtime-changes.html}, developer could resolve this kind of crashes by either (1) retaining a stateful object when the activity is recreated or (2) avoiding the activity recreation. We choose the first strategy because it is more flexible as it allows activity recreations instead of preventing the configuration changes altogether. Listing~\ref{lst:configexample} presents an example that explains how we retain the \texttt{Option} object by using the saved instance after the configuration changes to prevent null reference of the object (S2: Retain object).
\begin{lstlisting}[style=mystyle, escapechar=^,caption=Example of handling crashes during configuration changes,upquote=true,label={lst:configexample}]
public void onCreate(Bundle savedInstanceState) {
   super.onCreate(savedInstanceState);
+  setRetainInstance(true);// retain this fragment
}
// new field for saving the object
+ private static Option saveOption;

public View onCreateView(LayoutInflater inflater, ViewGroup container, Bundle savedInstanceState) {
// saving and loading the object
+  if(option!=null){  saveOption = option; }
+ else{ option = saveOption; }
  switch (option.getButtonStyle()) { //crashing point
\end{lstlisting}

\smallskip

\noindent\textbf{Commit transactions} Each fragment can be modified independently of the host activity by performing a set of changes. Each set of changes that we \emph{commit} (perform requested modifications atomically) to the activity is called a \emph{transaction}. Android documentation~\footnote{https://developer.android.com/reference/android/app/FragmentTransaction.html} specifies rules to prohibit committing transactions at certain stages of the lifecyle. Transactions that are committed in disallowed stages will cause the app to throw an exception. For example, invoking \texttt{commit()} after \texttt{onSaveInstanceState()} will lead to \texttt{IllegalStateException} since the transaction could not be recorded during this stage. We employ two strategies for resolving the incorrect commits: (S6: Move stmt) moving \texttt{commit()} to a legal callback (e.g., onPostResume()), (S4: Replace method) replacing \texttt{commit()} with \texttt{commitAllowingStateLoss()}.

\smallskip

\noindent\textbf{Communication between activity and fragment} The lifecycle of a fragment is affected by the lifecycle of its host activity~\footnote{https://developer.android.com/guide/components/fragments.html}. 

==> backup/sprsummarytable.tex <==
\begin{table*}[!ht]
\centering
\caption{Overall Result on mSPR}
\label{spr-sum}
\scalebox{0.75}{
\begin{tabular}{|l|c|c||c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\multirow{3}{*}{Subjects}} & \multicolumn{2}{c||}{Same Patch} & \multicolumn{9}{c|}{Different Patch} \\ \cline{2-12} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\multirow{2}{*}{Subject}} & \multicolumn{1}{c||}{\multirow{2}{*}{Average Speedup}} & \multicolumn{2}{c|}{Similar to Human Patch} & \multicolumn{1}{c|}{\multirow{2}{*}{Delete Less}} & \multicolumn{2}{c|}{Better Condition} & \multicolumn{2}{c|}{Closer Location} & \multicolumn{1}{c|}{\multirow{2}{*}{No Repair}} & \multicolumn{1}{c|}{\multirow{2}{*}{Average Speedup}} \\ \cline{4-5} \cline{7-10}
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c||}{} & \multicolumn{1}{c|}{SPR} & \multicolumn{1}{c|}{mSPR} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{SPR} & \multicolumn{1}{c|}{mSPR} & \multicolumn{1}{c|}{SPR} & \multicolumn{1}{c|}{mSPR} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\ \hline
php & 12 & 2.09 & 0 & 1 & 1 & 0 & 2 & 0 & 0 & 0 & 1.81 \\
libtiff & 2 & 2.10 & 0 & 0 & 0 & 0 & 2 & 1 & 0 & 1 & 1.31 \\
python & 1 & 1.76 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 1.34 \\
gmp & 2 & 1.42 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1.42 \\
gzip & 1 & 1.08 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0.56 \\
wireshark & 3 & 1.52 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 2.78 \\
fbc & - & - & - & - & - & - & - & - & - & - & - \\
lighthttpd & 0 & 0.00 & 0 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2.37 \\\hline
%Total/Average & 21 & 1.25 & 0 & 2 & 3 & 0 & 9 & 1 & 0 & 1 & 1.45
Total/Average & \sprTotSame & \sprTotSpeedSame &0& \sprTotSimilar & \sprTotDel & 0 &\sprTotLoc & \sprTotNoRep &0 & \sprTotNoRep & \sprTotSpeed\\ \hline

\end{tabular}
}
\end{table*}


==> sections/motivating_example.tex <==
\section{Motivating Example}
\modifyhaibo{
As shown in Figure 2, we use two types of simplification, ``Use API'' and ``Replace with annotations'' as our motivating examples to illustrate the benefits of our study and tool for program simplification, compared to classical program reduction and the program slicing techniques.

In Figure 2a, a chunk of code is replaced with ...

}
